Adversarial Perturbations Against Real-Time Video Classification Systems

Recent research has demonstrated the brittleness of machine learning systems to adversarial perturbations. However, the studies have been mostly limited to perturbations on images and more generally, classification that does not deal with temporally varying inputs. In this paper we ask "Are adversarial perturbations possible in real-time video classification systems and if so, what properties must they satisfy?" Such systems find application in surveillance applications, smart vehicles, and smart elderly care and thus, misclassification could be particularly harmful (e.g., a mishap at an elderly care facility may be missed). We show that accounting for temporal structure is key to generating adversarial examples in such systems. We exploit recent advances in generative adversarial network (GAN) architectures to account for temporal correlations and generate adversarial samples that can cause misclassification rates of over 80% for targeted activities. More importantly, the samples also leave other activities largely unaffected making them extremely stealthy. Finally, we also surprisingly find that in many scenarios, the same perturbation can be applied to every frame in a video clip that makes the adversary's ability to achieve misclassification relatively easy.

==> CCS-Sasha 2/abs2.tex <==
\begin{abstract}
{
Recent research has demonstrated the brittleness of machine learning systems
to adversarial perturbations. However, the studies have been mostly limited to
perturbations on images and more generally, classification that does not deal
with temporally varying inputs. In this paper we ask "Are adversarial perturbations
possible in real-time video classification systems and if so, what properties must
they satisfy?" Such systems find application in surveillance applications, smart vehicles,
and smart elderly care 
and thus,
misclassification could be particularly harmful (e.g., a mishap at an elderly
care facility may be missed). We show that accounting for temporal
structure is key to generating adversarial examples in such systems. We exploit
recent advances in generative adversarial network (GAN) architectures to account for
temporal correlations and generate adversarial samples that can cause misclassification
rates of over 80 \% for targeted activities. More importantly, the samples also leave
other activities largely unaffected making them extremely stealthy. Finally, we also surprisingly
find that in many scenarios, the same perturbation can be applied to every frame in a video clip that makes
the adversary's ability to achieve misclassification relatively easy.
}
\end{abstract}


\begin{comment}
   { 
    - Recent research studies have reported that machine learning systems vulnerable to aptly generated adversarial perturbations. 
    - attack vectors are mostly analyzed in image space, and have shown image-agnostic adversarial attacks are possible
    - There are several challenges to directly import image space work to video space
    - To this end, this is the first work on video space
    - We show that the perturbations produced on image space do not work on video, as video classification relies on temporal relationship among the frames
    - To attack such systems is challenging
    - We propose a GAN architecture to model perturbations
    - On top of that, we are not only misclassifying  a action, but also misclassifying it to a target class
    - We analyze several possible perturbations that we can add to misclassify video
    - We present the results.
\end{abstract}
}
\end{comment}


==> CCS-Sasha 2/authors.tex <==
\author{Shasha Li}
\affiliation{%
\institution{University of California, Riverside}
  \city{Riverside}
  \state{California}
}
\email{sli057@ucr.edu}

\author{Ajaya Neupane}
\affiliation{%
  \institution{University of California, Riverside}
  \city{Riverside}
  \state{California}
}
\email{ajaya@ucr.edu}

\author{Sujoy Paul}
\affiliation{%
  \institution{University of California, Riverside}
  \city{Riverside}
  \state{California}
}
\email{spaul003@ucr.edu}

\author{Chengyu Song}
\affiliation{%
  \institution{University of California, Riverside}
  \city{Riverside}
  \state{California}
}
\email{csong@cs.ucr.edu}

\author{Srikanth V. Krishnamurthy}
\affiliation{%
  \institution{University of California, Riverside}
  \city{Riverside}
  \state{California}
}
\email{krish@cs.ucr.edu}

\author{Amit K. Roy Chowdhury}
\affiliation{%
  \institution{University of California, Riverside}
  \city{Riverside}
  \state{California}
}
\email{amitrc@ece.ucr.edu}

\author{Ananthram Swami}
\affiliation{%
  \institution{United States Army Research Laboratory}
}
\email{ananthram.swami.civ@mail.mil}
% The default list of authors is too long for headers.
\renewcommand{\shortauthors}{S. Li et al.}


==> CCS-Sasha 2/back2.tex <==
\section{Background}

In this section, we provide the background relevant to our work. Specifically, we discuss how a real-time video classification system works and what standard algorithms are currently employed for action recognition. We also discuss generative adversarial networks (GANs) in brief. 
%{\color{green} We also provide a brief overview on the data-sets we chose for validating our attack models. Need to move this and threat model to another section.}

\subsection{Real-time video-based classification systems}
\label{sec:var}

\begin{comment}
\reminder{Sasha:I think we need specify our attack targets \textbf{real-time} system. 
This need to be mentioned in both abstract and introduction, like, 
for the introduction part, maybe more story on \textbf{real-time application}}
\end{comment}
%{\color{red}\{comment from Shasha, I think this part is more suitable for introducation\}}

DNN based video classification systems are being increasingly deployed in real-world scenarios. 
Examples include fall detection in elderly care \cite{foroughi2008intelligent}, abnormal event 
detection on campuses \cite{umboocv2017caseNCHU,umboocv2017caseTai}, 
security surveillance for smart cities \cite{umboocv2017caseCBS}, and self-driving cars \cite{kataoka2018temporal,kataoka2018drive}. 
Given an input real-time video stream, which may contain one or more known actions,
the goal of a video classification system is to correctly recognize the sequence of the
performed actions. Real-time video classification systems commonly use a {\em sliding window} 
to analyze a video stream \cite{fanello2013one,tripathi2016real}. 
The classifier computes an output score for each class in each
sliding window. 
The sliding window moves with a stride. 
%, maybe fixed or dynamic\cite{tripathi2016real}. {\color{red} Do you mean: The sliding window moves in steps, either crossing a fixed number or dynamic number of frames at each step?} \reminder{yes}
Moving in concert with the sliding window, one can generate ``score curves'' for each 
action class. Note that the scores for all the action classes evolve with time. The score curves are then smoothed (to remove noise) as shown in \autoref{fig:real_time}. With the smoothed score curves, 
the on-going actions are predicted online.
From the figure one can see that, the real-time video classification system is fooled if one can make the classifier output a low score for the true class in each sliding window; with this, the true actions will not 
be recognized.
\begin{figure}[!ht]
    \centering
    \includegraphics[scale=.36]{images/real_time_system.png}
    \caption{This figure \cite{fanello2013one} illustrates the score curves computed by a video classifier with a sliding window for every class. Real-time video classification systems use these score curves to do online action recognition. }
    \label{fig:real_time}
\end{figure}


%We present the development of classifiers used for action recognition and show the state-of-art C3D classifier\cite{tran2015learning} in detail, which is what we attack in the paper. .

%To be more specific, a classifier takes a sequence of frames, then generates classification score for them, and move to the next sequence of frames. This results in a score curve which evolves with time. The classifier here we use is C3D, which is a state-of-art model \autoref{sec:c3d}.

\begin{figure*}[!ht]
	\centering
	\includegraphics[scale=.36]{images/C3D.png}
	\caption{The C3D architecture\cite{tran2015learning}.
	C3D net has 8 convolution, 5 max-pooling, and 2 fully connected layers, followed by a softmax output layer. All 3D convolution kernels are $3 \times 3 \times 3$ with a stride \cite{tran2015learning} of 1 in both spatial and temporal dimensions. The number of filters are shown in each box. The 3D pooling layers are represented from pool1 to pool5. All pooling kernels are $2 \times 2 \times 2$, except for pool1, which is $1 \times 2 \times 2$. Each fully connected layer has 4096 output units.}
	\label{fig:c3d}
\end{figure*}

\subsection{The C3D classifier}\label{sec:c3d} 

Next, %we describe the classifiers used in video-based action recognition. In particular,
we describe what is called the C3D classifier~\cite{tran2015learning}, a state of the art
classifier that we target in our paper. 

\begin{comment}
{
Action classification has been studied by the computer vision community for decades. 
Once a good representation is provided, it is generally assumed that 
classification is easy. 
Therefore, a considerable proportion of recent efforts focus on video representation. 
Video representation presents unique challenges due to the fact that 
video consists of motion features in addition to the spatial features present in 2D images. 
Handling motion calls for more complex architectures and, often, 
adds higher memory and computational demands.
Hand-crafted representations such as SIFT-3D\cite{scovanner20073}, HOG3D\cite{klaser2008spatio}, and improved iDT\cite{wang2013action} were popular before the 
emergence of Deep Neural Networks (DNNs).

With the availability of powerful parallel machines (GPUs, CPU clusters), and  large amount of training data, DNNs bring another boost on video feature learning, among which spatio-temporal networks\cite{karpathy2014large,tran2015learning,varol2017long} and two-stream networks\cite{carreira2017quo,simonyan2014two} outperform other network structures\cite{herath2017going,gu2017recent}. Without non-trivial pre-processing on the video stream, spatio-temporal CNN,like \cite{tran2015learning} shows their efficiency and effectiveness, among which C3D is the start-of-art one\cite{gu2017recent}.
}
\end{comment}

DNNs and in particular convolutional neural networks (CNNs) are being increasingly applied in video 
classification.
%~\cite{karpathy2014large,tran2015learning,varol2017long,karpathy2014large,tran2015learning,varol2017long}. 
Among these, spatio-temporal networks like C3D \cite{tran2015learning} and two-stream networks like I3D \cite{carreira2017quo} outperform other network structures\cite{herath2017going,gu2017recent}. 
Without the requirement of non-trivial pre-processing on the video stream, 
spatio-temporal networks demonstrate high efficiency; among these, C3D is the start-of-art model~\cite{gu2017recent}.
 
%Among these, the C3D model\cite{tran2015learning} is   
%arguably one of the most popular architectures \cite{herath2017going,gu2017recent}. 
%This is because the 
The
C3D model is generic, which means that it can differentiate across different types of videos (e.g., videos of actions in sports, actions involving pets, actions relating to food etc.). 
It also provides a compact representation that facilitates scalability in processing, storage, and retrieval. It is also extremely efficient in classifying video streams
(needed in real-time systems).

\begin{comment}
{
1) \textbf{generic}, so that it can represent different types of videos well while being discriminate. Using human action recognition as an example, videos can include spots, food, pet and so on; 2) \textbf{compact}, as we are working on streams of videos, a compact descriptor helps processing, storing and retrieving tasks much more scalable; 3) \textbf{efficient} to compute, as thousands of videos are expected to be processed every minute in real world systems.
}
\end{comment}

Given its desirable attributes and popularity, without loss of generality, 
we use the C3D model as our attack target in this paper.
The C3D model is based on 3D ConvNet (a 3D CNN) \cite{karpathy2014large,tran2015learning,varol2017long}, which is very effective in modeling 
temporal information 
(because it employs 3D convolution and 3D pooling operations). 

The architecture and hyperparamters of C3D are shown in \autoref{fig:c3d}. The input to the C3D 
classifier is a clip consisting of 16 consecutive frames. This means that upon using C3D, 
the sliding window size is 16. Both the height and the width of each frame are 112 
pixels and each frame has 3 (RGB) channels. 
The last layer of C3D is a softmax layer that provides a classification score 
with respect to each class.


%-describe common network settings
%I3D is more advanced version \cite{carreira2017quo}

\begin{comment}
{
\subsection{Datasets}\label{sec:dataset}

\subsubsection{UCF 101}
UCF 101 dataset used in our experiments is the standard dataset collected from youtube which includes 13320 videos from 101 human action categories \cite{soomro2012ucf101}. The videos collected in this dataset have variations in camera motion, appearance, background, illumination conditions etc. Given the diversity it provides, we considered the dataset to validate the feasibility of our attack model on the videos. 

\subsubsection{Jester}

The 20BN-JESTER dataset (JESTER) \cite{jester2016} is a recently collected dataset with gesture videos. These videos are recorded by crowd-source workers performing 27 kinds of gestures such as "Thumbing up", "Swiping Left", and "Turning hand counterclockwise". We use this dataset to validate our attack model on a fine-defined action set videos.
Since this dataset does not provide the label for the testing set right now, we use the validation set as our testing set, and split 1400 inputs from training set as our validation set.
}
\end{comment}

\subsection{Generative Adversarial Networks and their relevance}
\label{sec:nag}

Generative Adversarial Networks (GANs) \cite{goodfellow2014generative} 
were initially developed to generate synthetic content (and in particular, images) that conformed
with the space of natural content~\cite{zhu2016generative,huang2017stacked}. Recently,
there has also been work on using GANs for generating synthetic videos~\cite{vondrick2016generating}.
The GAN consists of two components viz., a generator or generative model that tries to learn
the training data distribution and a discriminator or discriminative model that seeks to 
distinguish the generated distribution from the training data distribution. 

To elaborate, consider the use of a GAN for video generation. An archtecture for this purpose is
shown in \autoref{fig:gan_arc}. The generator $G$, learns a map 
from a random vector $z$ in latent space, to a natural video clip $V$; in other words, $G(z)=V$, where $z$ is usually sampled from a simple distribution such as a Gaussian distribution ($N(0,1)$)
or a uniform distribution ($U(-1,1)$). The discriminator $D$ takes a video clip as input
(either generated or natural),
and outputs the probability that it is from the training data (i.e., the probability that
the video clip is natural).
The interactions between $G$ and $D$ are modeled as a game and in theory, at the end $G$ must be able to generate video clips from the true training set distribution. 

Recently, a GAN-like architecture has been used to generate adversarial perturbations on images \cite{mopuri2017nag} .
The authors of ~\cite{mopuri2017nag} keep a trained discriminator fixed; 
its goal is to classify the inputs affected by the perturbations from the
generator. The generator learns from the discriminator classifications to modulate its perturbations.
Similarly,  we apply the GAN-like architecture wherein
the objective is to allow the generator to learn a distribution for candidate perturbations that can
fool our discriminator. Our model incorporates significant extensions to the GAN structure
used in \cite{mopuri2017nag} to account for the unique properties of video classification that
were discussed earlier. 


\begin{comment}
{
as a popular generative model, has been commonly used to mdoel the space of natural images\cite{zhu2016generative,huang2017stacked}, and recently even videos\cite{vondrick2016generating}, thus generate human-craft natural images and videos. GAN consists of two models: a generative model G that try to learn the training data distribution, and a disriminative model D that try to disingush the train data distribution and the genrated distribution.
To be more specific, The geneartor G learns a map from a random vector $z$ in latent space to a natural image $I$; i.t., $G(z)=I$, where $z$ is usually sampled from a simple distribution (e.g.,$N(0,1),U(-1,1)$). The discrimiatr D accpets an image and outputs the probablity for it coming from the training data ranther than G.
Posing the training process as a game between G and D, the two models are trained simitanioly and at the end (in theory) G exactly reprocudes the true data distribution and the D guesses at random, unable to find a difference. The archtecture is present in \autoref{fig:gan_arc}. There are usually two objectives for genertor 1) fool the discriminator; 2) explore the space, which also means generate diverse natural image.
}
\end{comment}

\begin{comment}
{
Our work based on GAN and try to model the distribution of candidate perturbations. However, we concentrate more on fooling the discriminator, and do not make extra effects to explore diverse perturbations. \cite{mopuri2017nag} in image area is the most related work in the sense that we both use GAN structure. However, their model is build on 2D system and are more concentrate on the diversity part. In addition, we add a new process part between the generator and the discriminator to help overcome the unique challegnes in attacking real-time  system. We present the overview of our archectecture in \autoref{fig.our_arc}. The parts inclued in the dotted line are presented further in \autoref{sec:sec_tac}.
}
\end{comment}


\begin{comment}
{\color{red}There is one work using generatvie way to generate perturbatons. others are kind of based on reconstruction}
{\color{blue}{\textbf{need to explain NAG further here} Generative Models \cite{goodfellow2014generative} have been commonly used by researchers to mdoel the space of natural images and thus generate human-craft natural images.
natural images 
perturbations for images \cite{moosavi2017universal,mopuri2017nag}. 

The generative model can learn from the training data and produce an an image inconspicuous to the original one. In this work, use adversarial generative network to produce perturbations which can be added to the videos to fool the recognition system. }}
\end{comment}
%The 20BN-JESTER dataset is a large collection of densely-labeled video clips that show humans performing pre-definded hand gestures in front of a laptop camera or webcam. The dataset was created by a large number of crowd workers. It allows for training robust machine learning models to recognize human hand gestures. It is available free of charge for academic research. Commercial licenses are available upon request








==> CCS-Sasha 2/conclusion.tex <==
\section{Conclusions}

In this paper, we investigate the problem of generating adversarial samples for attacking video classification systems. We identify three key challenges that will need to be addressed in order to generate such samples namely, generating perturbations in real-time, making the perturbations stealthy and accounting for the temporal structure of frames in a video clip. We exploit recent advances in GAN architectures, extending them significantly to solve these challenges and generate very potent adversarial samples against video classification systems. We perform extensive experiments on two different datasets one of which captures coarse-grained actions (e.g., applying make up) while the other captures fine-grained actions (hand gestures). We demonstrate that our approaches are extremely potent, achieving around 80 \% attack success rates in both cases. We also discuss possible defenses that we propose to investigate in future work.

%\section{Appendices}


==> CCS-Sasha 2/discussion.tex <==
\section{Discussion}

\heading{Black box attacks:}
In this work we assumed that the adversary is fully aware of the DNN being deployed
(i.e., white box attacks).
However, in practice the adversary may need to determine the type of
DNN being used in the video classification system,
and so a black box approach may be needed.
Given recent studies on the transferability of adversarial inputs~\cite{papernot2016transferability},
we believe black box attacks are also feasible.
We will explore this in our future work.

\heading{Context dependency:}
Second, the approach that we developed does not account for contextual information,
i.e., consistency between the misclassified result and the context.
For example, the context relates to a baseball game a human overseeing
the system may notice an inconsistency
when the action of hitting a ball is misclassified into applying makeup.
Similarly, because of context, if there is a series of actions that we want to misclassify,
inconsistency in the misclassification results
(e.g., different actions across the clips) may also raise an alarm.
For example, let us consider a case where the actions include running,
kicking a ball, and applying make up.
While the first two actions can be considered to be {\em reasonable}
with regards to appearing together in a video, the latter two are unlikely.
%This may trigger alerts.
Generating perturbations that are consistent with the context of the video
is a line of future work that we will explore and is likely to require
new techniques.
In fact, looking for consistency in context may be a potential defense,
and we will also examine this in depth in the future.

\heading{Defenses:}
{\color{black} In order to defense against the attacks against video classification systems,
one can try some existing defense methods in image area, such as feature squeezing \cite{xu2017feature1,xu2017feature2} and ensemble adversarial training \cite{tramer2017ensemble} (although their
effectiveness is yet unknown). Considering the properties of video that were discussed, 
we envision some exclusive defense methods for protecting video classification systems
below, which we will explore in future work.}

%In order to defend against the attacks against video classification systems,
One approach is to examine the consistency between the classification of
consecutive frames (considered as images) within a clip,
and between consecutive clips in a stream. %as a holistic entity.
A sudden change in the classification results could raise an alarm.
However, while this defense will work well in cases where the temporal flow
is not pronounced (e.g., the UCF101 dataset),
it may not work well in cases with pronounced temporal flows.
For example, with respect to the Jester dataset,
with just an image it may be hard to determine whether the hand is being moved right or left.

The second line of defense may be to identify an object that is present in the video,
e.g., a soccer ball in a video clip that depicts a kicking action.
We can use an additional classifier to identify such objects
in the individual frames that compose the video.
Then, we can look for consistency with regards to the action and the object,
e.g., a kicking action is can be associated with a soccer ball,
but cannot be associated with a make up kit.
Towards realizing this line of defense,
we could use existing image classifiers in conjunction with
the video classification system.
We will explore this in future work.


{\begin{comment}
{
In this section we summarize our findings and further discuss the study insights. 

\heading{Study Insights:} In this study, we empirically demonstrate that we can generate adversarial perturbations against the real-time video classification systems despite the challenges that we discussed. We introduce the concept of dual purpose perturbations, and use a GAN inspired framework to actually generate the circular and 2D-dual purpose perturbations. We observe the 2D-DUP performed as good as C-DUP in most cases, which is surprising as video consists of both spatial and temporal information, and 2D perturbations should not heavily affect the temporal information. On further analyzing our results on Jester dataset, we observe that 'sliding hand right' is mostly misclassified as 'sliding two fingers right' which has similar temporal information, with 2D-DUP. Btu when we attack 'shaking hand' video, 2D-DUP did not achieve good results since there is no other class that is temporally similar to shaking hand.This might mean that a model built to identify classes with similar temporal information might be more vulnerable to adversarial perturbations as affecting appearance may be enough to attack the videos. 


On analyzing the results from circular DUP in UCF101 we observed that 2D-DUP can achieve successful attack on every target set.  We observe that the frame of C-DUP look 

%--UCF101 , applying lipstick is also misclassifed to something else,  
%and we use 2D it works, its stil misclssified, we do not use temporal information. This implies that c3d may not use enough temporal information, it emphasize appearche information.

--Jester dataset, when we use shake hand, 2D cannot achieve a good attack, because that C3D model takes the temporal information into consideration. Also since there is no other class that is temporally similar to shaking hand, the attack is hard. 

%If we want our system to be robust, it is better to have less class, and no classes without similar temporal information. For example some one picking up a pen can be misclassified as someone picking up a book, which can harm the robustness of the system. 

--classifier is weak, temporal information...
-- model is not good, tries to recognize too many classes.
%-- There is a class that is temporally similar.

-basically we should keep the number of class to be as little as possible. This system does recognize senior falling, then just falling and not falling, then don't recognize other actions. Multiple information may may system more vulnerable. 

\reminder{insight: we need to carefully choose the dataset}

\heading{Open Question:} One of the important findings of our study is the existence of the dual-purpose perturbation. The common assumption is that adding perturbation on videos will misclassify everything, but we have shown that it can be configured such that it can only misclassify target classes. But why is an open ended question. Future works might be needed to explore more on the answer.

This can cause some target classes misclassify and non-target classes as is even when perturbation is applied on all clips. This is an open ended question.

\subsection{Possible Defenses}

-- get classification result on the randomly chose frame from the clip, and the clip itself to validate the results.
-- Patrick EuroS\&P paper
-- Transferability Paper
-- Wagner Paper

\subsection{Future Work}

--Transferability - related to blackbox attack.
--Right now we use universal perturbation, which can solve boundary problem. What if we do not generate an  universal perturbation, and just focus on a perturbation which evolves with the video frames. 


\subsection{Limitations}

-- generally for generator, we should have an object, for which it can generate diverse output.
-- since we are focusing on attack, we do not have that object. Previously we can get a space of perturbation which could achieve this attack, but in our study we saw that with different noise input, the generator tend to generate same perturbation. But for attack to be successful, even a single perturbation is enough.

-- We do not track activities across the videos
-- All experiments are done for single target classes, but it should be easy to extend it to multiple target classes

}
\end{comment}


==> CCS-Sasha 2/eval2.tex <==
\section{Evaluations}
\label{sec:evaluation}
In this section, we showcase the efficacy of the perturbations 
generated by our proposed approaches on both the UCF-101 and Jester datasets.

\begin{figure*}[t]
	\centering
	\begin{subfigure}{0.12\textwidth}
		\includegraphics[scale=.5]{images/3D_UP/perturbation_00.png}
	\end{subfigure}
	\begin{subfigure}{0.12\textwidth}
		\includegraphics[scale=.5]{images/3D_UP/perturbation_01.png}
	\end{subfigure}
	\begin{subfigure}{0.12\textwidth}
		\includegraphics[scale=.5]{images/3D_UP/perturbation_02.png}
	\end{subfigure} \vspace{0.01\textwidth}
	\begin{subfigure}{0.12\textwidth}
		\includegraphics[scale=.5]{images/3D_UP/perturbation_03.png}
	\end{subfigure}
	\begin{subfigure}{0.12\textwidth}
		\includegraphics[scale=.5]{images/3D_UP/perturbation_04.png}
	\end{subfigure}
	\begin{subfigure}{0.12\textwidth}
		\includegraphics[scale=.5]{images/3D_UP/perturbation_05.png}
	\end{subfigure}
	\begin{subfigure}{0.12\textwidth}
		\includegraphics[scale=.5]{images/3D_UP/perturbation_06.png}
	\end{subfigure}
	\begin{subfigure}{0.12\textwidth}
		\includegraphics[scale=.5]{images/3D_UP/perturbation_07.png} 
	\end{subfigure}
	\begin{comment}
	\begin{subfigure}{0.12\textwidth}
		\includegraphics[scale=.5]{images/3D_UP/perturbation_08.png}
	\end{subfigure}
	\begin{subfigure}{0.12\textwidth}
		\includegraphics[scale=.5]{images/3D_UP/perturbation_09.png} 
	\end{subfigure}
	\begin{subfigure}{0.12\textwidth}
		\includegraphics[scale=.5]{images/3D_UP/perturbation_10.png}
	\end{subfigure}
	\begin{subfigure}{0.12\textwidth}
		\includegraphics[scale=.5]{images/3D_UP/perturbation_11.png}
	\end{subfigure}
	\begin{subfigure}{0.12\textwidth}
		\includegraphics[scale=.5]{images/3D_UP/perturbation_12.png}
	\end{subfigure}
	\begin{subfigure}{0.12\textwidth}
		\includegraphics[scale=.5]{images/3D_UP/perturbation_13.png}
	\end{subfigure}
	\begin{subfigure}{0.12\textwidth}
		\includegraphics[scale=.5]{images/3D_UP/perturbation_14.png}
	\end{subfigure}
	\begin{subfigure}{0.12\textwidth}
		\includegraphics[scale=.5]{images/3D_UP/perturbation_15.png}
	\end{subfigure}
	\end{comment}
	\caption{DUP on UCF-101}
	\label{fig:v_DUP}
\end{figure*}


\begin{figure*}[t]
	\centering
	\begin{subfigure}{0.12\textwidth}
		\includegraphics[scale=.5]{images/3D_CUP/perturbation_00.png}
	\end{subfigure}
	\begin{subfigure}{0.12\textwidth}
		\includegraphics[scale=.5]{images/3D_CUP/perturbation_01.png}
	\end{subfigure}
	\begin{subfigure}{0.12\textwidth}
		\includegraphics[scale=.5]{images/3D_CUP/perturbation_02.png}
	\end{subfigure}
	\begin{subfigure}{0.12\textwidth}
		\includegraphics[scale=.5]{images/3D_CUP/perturbation_03.png}
	\end{subfigure} 	\vspace{0.01\textwidth}
	\begin{subfigure}{0.12\textwidth}
		\includegraphics[scale=.5]{images/3D_CUP/perturbation_04.png}
	\end{subfigure}
	\begin{subfigure}{0.12\textwidth}
		\includegraphics[scale=.5]{images/3D_CUP/perturbation_05.png}
	\end{subfigure}
	\begin{subfigure}{0.12\textwidth}
		\includegraphics[scale=.5]{images/3D_CUP/perturbation_06.png}
	\end{subfigure}
	\begin{subfigure}{0.12\textwidth}
		\includegraphics[scale=.5]{images/3D_CUP/perturbation_07.png}
	\end{subfigure} 
	\begin{comment}
	\begin{subfigure}{0.12\textwidth}
		\includegraphics[scale=.5]{images/3D_CUP/perturbation_08.png}
	\end{subfigure}
	\begin{subfigure}{0.12\textwidth}
		\includegraphics[scale=.5]{images/3D_CUP/perturbation_09.png}
	\end{subfigure}
	\begin{subfigure}{0.12\textwidth}
		\includegraphics[scale=.5]{images/3D_CUP/perturbation_10.png}
	\end{subfigure}
	\begin{subfigure}{0.12\textwidth}
		\includegraphics[scale=.5]{images/3D_CUP/perturbation_11.png}
	\end{subfigure}
	\begin{subfigure}{0.12\textwidth}
		\includegraphics[scale=.5]{images/3D_CUP/perturbation_12.png}
	\end{subfigure}
	\begin{subfigure}{0.12\textwidth}
		\includegraphics[scale=.5]{images/3D_CUP/perturbation_13.png}
	\end{subfigure}
	\begin{subfigure}{0.12\textwidth}
		\includegraphics[scale=.5]{images/3D_CUP/perturbation_14.png}
	\end{subfigure}
	\begin{subfigure}{0.12\textwidth}
		\includegraphics[scale=.5]{images/3D_CUP/perturbation_15.png}
	\end{subfigure}
	\end{comment}
	\caption{C-DUP on UCF-101%:  We observe that the middle crossing pattern evolves along frames as marked by red circles, the bar pattern marked by red rectangular evolves. Also the color of the bottom part is changing.
	}
	\label{fig:v_CUP}
\end{figure*}


\begin{figure*}[t]
	\centering
	\begin{subfigure}{0.12\textwidth}
		\includegraphics[scale=.5]{images/sliding/perturbation_00.png}
	\end{subfigure}
	\begin{subfigure}{0.12\textwidth}
		\includegraphics[scale=.5]{images/sliding/perturbation_01.png}
	\end{subfigure}
	\begin{subfigure}{0.12\textwidth}
		\includegraphics[scale=.5]{images/sliding/perturbation_02.png}
	\end{subfigure} \vspace{0.01\textwidth}
	\begin{subfigure}{0.12\textwidth}
		\includegraphics[scale=.5]{images/sliding/perturbation_03.png}
	\end{subfigure}
	\begin{subfigure}{0.12\textwidth}
		\includegraphics[scale=.5]{images/sliding/perturbation_04.png}
	\end{subfigure}
	\begin{subfigure}{0.12\textwidth}
		\includegraphics[scale=.5]{images/sliding/perturbation_05.png}
	\end{subfigure}
	\begin{subfigure}{0.12\textwidth}
		\includegraphics[scale=.5]{images/sliding/perturbation_06.png}
	\end{subfigure}
	\begin{subfigure}{0.12\textwidth}
		\includegraphics[scale=.5]{images/sliding/perturbation_07.png} 
	\end{subfigure}
	\begin{comment}
	\begin{subfigure}{0.12\textwidth}
		\includegraphics[scale=.5]{images/sliding/perturbation_08.png}
	\end{subfigure}
	\begin{subfigure}{0.12\textwidth}
		\includegraphics[scale=.5]{images/slidingd/perturbation_09.png} 
	\end{subfigure}
	\begin{subfigure}{0.12\textwidth}
		\includegraphics[scale=.5]{images/sliding/perturbation_10.png}
	\end{subfigure}
	\begin{subfigure}{0.12\textwidth}
		\includegraphics[scale=.5]{images/sliding/perturbation_11.png}
	\end{subfigure}
	\begin{subfigure}{0.12\textwidth}
		\includegraphics[scale=.5]{images/sliding/perturbation_12.png}
	\end{subfigure}
	\begin{subfigure}{0.12\textwidth}
		\includegraphics[scale=.5]{images/sliding/perturbation_13.png}
	\end{subfigure}
	\begin{subfigure}{0.12\textwidth}
		\includegraphics[scale=.5]{images/sliding/perturbation_14.png}
	\end{subfigure}
	\begin{subfigure}{0.12\textwidth}
		\includegraphics[scale=.5]{images/sliding/perturbation_15.png}
	\end{subfigure}
	\end{comment}
	\caption{C-DUP on Jester for $T_1 = \{\text{slding hand right}\}$}
	\label{fig:sliding_visual}
\end{figure*}


\begin{figure*}[t]
	\centering
	\begin{subfigure}{0.12\textwidth}
		\includegraphics[scale=.5]{images/shakehand/perturbation_00.png}
	\end{subfigure}
	\begin{subfigure}{0.12\textwidth}
		\includegraphics[scale=.5]{images/shakehand/perturbation_01.png}
	\end{subfigure}
	\begin{subfigure}{0.12\textwidth}
		\includegraphics[scale=.5]{images/shakehand/perturbation_02.png}
	\end{subfigure} \vspace{0.01\textwidth}
	\begin{subfigure}{0.12\textwidth}
		\includegraphics[scale=.5]{images/shakehand/perturbation_03.png}
	\end{subfigure}
	\begin{subfigure}{0.12\textwidth}
		\includegraphics[scale=.5]{images/shakehand/perturbation_04.png}
	\end{subfigure}
	\begin{subfigure}{0.12\textwidth}
		\includegraphics[scale=.5]{images/shakehand/perturbation_05.png}
	\end{subfigure}
	\begin{subfigure}{0.12\textwidth}
		\includegraphics[scale=.5]{images/shakehand/perturbation_06.png}
	\end{subfigure}
	\begin{subfigure}{0.12\textwidth}
		\includegraphics[scale=.5]{images/shakehand/perturbation_07.png} 
	\end{subfigure}
	\begin{comment}
	\begin{subfigure}{0.12\textwidth}
		\includegraphics[scale=.5]{images/shakehand/perturbation_08.png}
	\end{subfigure}
	\begin{subfigure}{0.12\textwidth}
		\includegraphics[scale=.5]{images/shakehand/perturbation_09.png} 
	\end{subfigure}
	\begin{subfigure}{0.12\textwidth}
		\includegraphics[scale=.5]{images/shakehand/perturbation_10.png}
	\end{subfigure}
	\begin{subfigure}{0.12\textwidth}
		\includegraphics[scale=.5]{images/shakehand/perturbation_11.png}
	\end{subfigure}
	\begin{subfigure}{0.12\textwidth}
		\includegraphics[scale=.5]{images/shakehand/perturbation_12.png}
	\end{subfigure}
	\begin{subfigure}{0.12\textwidth}
		\includegraphics[scale=.5]{images/shakehand/perturbation_13.png}
	\end{subfigure}
	\begin{subfigure}{0.12\textwidth}
		\includegraphics[scale=.5]{images/shakehand/perturbation_14.png}
	\end{subfigure}
	\begin{subfigure}{0.12\textwidth}
		\includegraphics[scale=.5]{images/shakehand/perturbation_15.png}
	\end{subfigure}
	\end{comment}
	\caption{C-DUP on Jester for $T_2 = \{\text{shaking hand}\}$}
	\label{fig:shake_visual}
\end{figure*}




\subsection{Experimental Setup}
\label{sec:exptdesc}
%in attacking state-of-the-art algorithms (see \ref{sec:classifiers}) in video recognition systems. %We use two publicly available datasets (see \ref{sec:datasets} to physically realize our attacks.
%We choose uniform distribution $U[-1,1]$ as the latent space for the generator, which means we sampled random vectors from the  uniform distribution $U[-1,1]$,
\heading{Discriminator set-up for our experiments:}
We used the C3D classifier as our discriminator.
To set up the discriminator for our experiments,
we pre-train the C3D classifier as described in \S \ref{sec:realtime}.
The discriminator is then used to train our generator.
For our experiments on the UCF101 dataset,
we use the C3D model available in the Github repository \cite{c3dgit}.
This pre-trained C3D model achieves an average clip classification
accuracy of $96.1\%$ on the UCF101 dataset in benign settings
(i.e., no adversarial inputs).

For the experiments on the Jester dataset,
we fine-tune the C3D model from the Github repository \cite{c3dgit}.
First, we change the output size of the last fully connected layer to 27,
since there are 27 gesture classes in Jester.
We use a learning rate with exponential decay \cite{zeiler2012adadelta} to train the model.
The starting learning rate for the last fully connected layer is set to be $10^{-3}$
and $10^{-4}$ for all the other layers.
The decay step is set to 600 and the decay rate is 0.9.
The fine-tuning phase is completed in 3 epochs and
we achieve a clip classification accuracy of $90.03\%$ in benign settings.

\heading{Generator set-up for our experiments:}
For building our generators, we refer to the generative model used by
Vondrik \etal \cite{vondrick2016generating},
which has 3D de-convolution layers.

For generators for both C-DUP and 2D-DUP,
we use five 3D de-convolution layers \cite{biggs20103d}.
The first four layers are followed by a batch normalization \cite{ioffe2015batch}
and a $ReLU$ \cite{nair2010rectified} activation function.
The last layer is followed by a $tanh$ \cite{kalman1992tanh} layer.
The kernel size for all 3D de-convolutions is set to be $3\times 3\times 3$.
To generate 3D perturbations (i.e., sequence of perturbation frames),
we set the kernel stride in the C-DUP generator to 1 in both
the spatial and temporal dimensions for the first layer,
and 2 in both the spatial and temporal dimensions for the following 4 layers.
To generate a single-frame 2D perturbation,
the kernel stride in the temporal dimension is set to 1
(i.e., 2D deconvolution) for all layers in the 2D-CUP generator,
and the spatial dimension stride is 1 for the first layer and 2 for the following layers.
The numbers of filters are shown in brackets in
\autoref{fig:arc_roll} and \autoref{fig:arc_tile}.
The input noise vector for both generators are sampled from a uniform distribution $U[-1,1]$
and the dimension of the noise vector is set to be 100.
For training both generators, we use a learning rate with exponential decay.
The starting learning rate is 0.002.
The decay step is 2000 and the decay rate is 0.95.
Unless otherwise specified, the weight balancing the two objectives,
i.e., $\lambda$, is set to 1 to reflect equal importance between
misclassifying the target class and retaining the correct
classification for all the other (non-target) classes.

\heading{Technical Implementation}:
All the models are implemented in TensorFlow~\cite{abadi2016tensorflow}
with the Adam optimizer \cite{kingma2014adam}.
Training was performed on 16 Tesla K80 GPU cards with the batch size set to 32.

\heading {Dataset setup for our experiments:}
On the UCF-101 dataset (denoted UCF-101 for short),
different sets of target class $T$ are tested.
We use $T=\{\text{apply lipstick}\}$ for presenting the results in the paper.
Experiments using other target sets also yield similar results.
UCF-101 has 101 classes of human actions in total.
The target set $T$ contains only one class while
the ``non-target'' set $S=X-T$ contains 100 classes.
The number of training inputs from the non-target classes is
approximately 100 times the number of training inputs from the target class.
Directly training with UCF-101 may cause a problem due to the imbalance
in the datasets containing the target and non-target classes \cite{longadge2013class}.
Therefore, we under-sample the non-target classes by a factor of 10.
Further, when loading a batch of inputs for training,
we fetch half the batch of inputs from the target set and
the other half from the non-target set in order to balance the inputs.

For the Jester dataset, we also choose different sets of target classes.
We use two target sets $T_1=\{\text{sliding hand right}\}$ and
$T_2=\{\text{shaking hands} \}$ as our representative examples
because they are exemplars of two different scenarios.
Since we seek to showcase an attack on a video classification system,
we care about how the perturbations affect both the appearance information
and temporal flow information, especially the latter.
For instance, the `sliding hand right' class has
a temporally similar class `sliding two fingers right;'
as a consequence, it may be easier for attackers to cause clips in the former class
to be misclassified as the later class
(because the temporal information does not need to be perturbed much).
On the other hand, `shaking hands' is not temporally similar to any other class.
Comparing the results of these two target sets could provide some
empirical evidence on the impact of the temporal flow on our perturbations.
% a sense of
Similar to UCF-101, the number of inputs from the non-target classes is
around 26 times the number of inputs from the target class
(since there are 27 classes in total and we only have one target class
in each experiment).
%{\color{blue} I thought we have two target classes}
So we under-sample the non-target inputs by a factor of 4.
We also set up the environment to load half of the inputs from the
target set and the other half from the non-target set, in every batch.

\begin{figure*}[t]
	\centering
	\begin{subfigure}{0.4\textwidth}
		\includegraphics[scale=.4]{images/DUP_C_DUP_1.png}
		\caption{Attack success rate on UCF-101 for target class \\ 'applying lipstick'}
		\label{fig:ucf_target}
	\end{subfigure}
	\hspace{1mm}
	\begin{subfigure}{0.4\textwidth}
		\includegraphics[scale=.4]{images/DUP_C_DUP_2.png}
		\caption{Attack success rate on UCF-101 for other non-target classes (all except 'applying lipstick')}
		\label{fig:ucf_non}
	\end{subfigure}
\hspace{1mm}
	\begin{subfigure}{0.4\textwidth}
        \includegraphics[scale=.2]{images/sliding_right_target_acc.png}
        \caption{Attack success rate on Jester for target class \\ 'sliding hands right'}
        \label{fig:sliding_target}
    \end{subfigure}
\hspace{1mm}
    \begin{subfigure}{0.4\textwidth}
        \includegraphics[scale=.2]{images/sliding_right_non_acc.png}
        \caption{Attack success rate on Jester for non-target classes (all excepet 'sliding right')}
        \label{fig:sliding_non}
    \end{subfigure}
\hspace{1mm}
    \begin{subfigure}{0.4\textwidth}
        \includegraphics[scale=.2]{images/shake_target_acc.png}
        \caption{Attack success rate on Jester for target class \\ 'shaking hand'}
        \label{fig:shake_target}
    \end{subfigure}
\hspace{1mm}
    \begin{subfigure}{0.4\textwidth}
        \includegraphics[scale=.2]{images/shake_non_acc.png}
        \caption{Attack success rate on Jester for non-target classes (all except 'shaking hand')}
        \label{fig:shake_non}
    \end{subfigure}
    \caption{attack success rate for DUP and C-DUP}
\end{figure*}

\vspace{-0.07in}
\heading{Metrics of interest:}
For measuring the efficacy of our perturbations, we consider two metrics.
\textit{First,} the perturbations added on the videos should be quasi-imperceptible.
\textit{Second}, the attack success rate for the target and the non-target classes should be high.
We define attack success rates as follows:

\squishlist
	\item The attack success rate for the target class is the misclassification rate;
	\item the attack success rate for the other classes is the correct classification rate.
\squishend

\subsection{C-DUP Perturbations}
\label{eval:cdup}

In this subsection, we discuss the results of the C-DUP perturbation attack.
We use the universal perturbations (UP) and DUP perturbations as our baselines.
%We first show the perturbations generated by C-DUP and DUP, and then discuss the attack success rate.

\vspace{1mm}
\subsubsection{Experimental Results on UCF101}~
\vspace{-2mm}

\heading{Visualizing the perturbation:}
The perturbation clip generated by the DUP model is shown in \autoref{fig:v_DUP} and
the perturbation clip generated by C-DUP model is shown in \autoref{fig:v_CUP}.
The perturbation clip has 16 frames, and we
represent a visual representation of the first 8 frames for illustration\footnote{The complete 16-frame perturbation clips are shown in an appendix.}
We observe that the perturbation from DUP manifests an obvious disturbance among the frames.
With C-DUP, the perturbation frames look similar,
which implies that C-DUP does not perturb the temporal information by much, in UCF101.
%, but are actually slightly different from each other. For example, the middle crossing pattern (as marked by red circles), and the bar pattern (as marked by red rectangles) evolve, and the color of the bottom part is changing. {\color{red} I really don't understand the purpose of this. What are we trying to convey?}

\heading{Attack success rates:}
Recalling the discussion in \S \ref{sec:perturbframe}, one can expect that UP would cause inputs 
from the target class to be misclassified, but also significantly affect the correct classification 
of the other non-target inputs. On the other hand, oue would expect that DUP would achieve a stealthy attack, which would not cause much effect on the classification of non-target classes.

Based on the discussion in  \S \ref{sec:temporal},
we expect that DUP would work well when the perturbation clip is
well-aligned with the start point of each input clip to the classifier;
%(i.e., the sliding window is synchronized with the perturbation clips that are generated)
and the attack success rate would degrade as the misalignment increases.
We expect C-DUP would overcome this boundary effect and provide a better
overall attack performance (even with temporal misalignment).

We observe that when one considers no misalignment, DUP achieves a target misclassification rate
of 84.49 \%, while the non-target classes are correctly classified with a rate of 88.03 \%.
In contrast, when UP achieves a misclassification rate of 84.01 \% for the target class, only
45.2 \% of the other classes are correctly classified.
Given UP's inferior performance, we do not consider it any further in our evaluations.

The attack success rates with DUP and C-DUP, on the UCF-101 test set,
are shown in \autoref{fig:ucf_target} and \autoref{fig:ucf_non}.
The $x$ axis is the misalignment between perturbation clip and
and the input clip to the classifier. 
%{\color{blue} When there is no misalignment, we see the DUP can misclassify $84.49\%$ of inputs from target class 'applying lipstick' and leave $88.03\%$ of the other inputs classified correctly. We observe with UP, when it misclassifies $84.01\%$ inputs from target class, it leaves only $45.2\%$ of the other inputs correctly classified. }
% (recall the discussion on \autoref{fig:mismatch})
\autoref{fig:ucf_target} depicts the average misclassification rate for inputs from the target class.
We observe that when there is no misalignment, the attack success rate with the DUP is $84.49\%$,
which is in fact slightly higher than C-DUP.
However, the attack success rate with C-DUP is significantly higher
when there is misalignment.
Furthermore, the average attack success rate across all alignments for the target class with C-DUP is $84\%$,
while with DUP it is only $68.26\%$.
This demonstrates that C-DUP is more robust against boundary effects.
%Thus, C-DUP guarantees a high attack success rate with all different offsets.

\autoref{fig:ucf_non} shows that, with regards to the classification of inputs from
the non-target classes, C-DUP also achieves a performance slightly better than DUP
when there is mismatch.
The average attack success rate (across all alignments) with C-DUP is $87.52\%$ here,
while with DUP it is $84.19\%$.
%The rates are similar \reminder{because in both cases, we try to make the perturbation stealthy}.

\begin{comment}
{
\begin{figure*}[!ht]
    \centering
    \begin{subfigure}{0.3\textwidth}
        \includegraphics[scale=0.60]{images/2d_family/perturbation_00.png}
        \subcaption{UCF101 }
        \label{fig:2D_ucf}
    \end{subfigure}
    \begin{subfigure}{0.3\textwidth}
        \includegraphics[scale=0.60]{images/Jester-2D/perturbation_00.png}
        \subcaption{Jester $T_1$ }
        \label{fig:2D_jester_t1}
    \end{subfigure}
    \begin{subfigure}{0.3\textwidth}
        \includegraphics[scale=0.60]{images/perturbation_00_2.png}
        \subcaption{Jester $T_2$ }
        \label{fig:2D_jester_t2}
    \end{subfigure}
    \caption{2D-DUP visualization}
	\label{fig:2D_DUP}
\end{figure*}
}
\end{comment}

\begin{figure*}[t]
    \centering
    \begin{subfigure}{0.19\textwidth}
        \includegraphics[scale=.7]{images/2d_family/orginal_00.png}
    \end{subfigure}
    \begin{subfigure}{0.19\textwidth}
        \includegraphics[scale=.7]{images/2d_family/orginal_01.png}
    \end{subfigure}
    \begin{subfigure}{0.19\textwidth}
        \includegraphics[scale=.7]{images/2d_family/orginal_02.png}
    \end{subfigure}
    \begin{subfigure}{0.19\textwidth}
        \includegraphics[scale=.7]{images/2d_family/orginal_03.png}
    \end{subfigure}\vspace{0.02\textwidth}
    \begin{subfigure}{0.19\textwidth}
        \includegraphics[scale=.7]{images/2d_family/orginal_04.png}
    \end{subfigure}
    \begin{subfigure}{0.19\textwidth}
        \includegraphics[scale=.7]{images/2d_family/perturbed_img_00.png}
    \end{subfigure}
    \begin{subfigure}{0.19\textwidth}
        \includegraphics[scale=.7]{images/2d_family/perturbed_img_01.png}
    \end{subfigure}
    \begin{subfigure}{0.19\textwidth}
        \includegraphics[scale=.7]{images/2d_family/perturbed_img_02.png}
    \end{subfigure}
    \begin{subfigure}{0.19\textwidth}
        \includegraphics[scale=.7]{images/2d_family/perturbed_img_03.png}
    \end{subfigure}
    \begin{subfigure}{0.19\textwidth}
        \includegraphics[scale=.7]{images/2d_family/perturbed_img_04.png}
    \end{subfigure}
    \caption{Visualizing images after adding 2D dual purpose universal perturbation: Original frames are displayed in the first row and perturbed frames are displayed in the second row. The perturbation added to the frames in the second row is mostly imperceptible to the human eye.}
    \label{fig:2D_CUP}
\end{figure*}




\vspace{1mm}
\subsubsection{Experimental Results on Jester}~
\vspace{-2mm}

\heading{Visualizing the perturbation:}
Visual representations of the C-DUP perturbations for the two target sets,
$T_1=\{\text{sliding hand right}\}$ and $T_2=\{\text{shaking hands} \}$
are shown in  \autoref{fig:sliding_visual} and \autoref{fig:shake_visual}.
%{\color{red} which are fake ones right not, need to be substitute, but the trend should be similar}. 
We notice that compared to the perturbation
generated on UCF-101 (see \autoref{fig:v_CUP}).
there is a more pronounced evolution with respect to Jester
(see \autoref{fig:sliding_visual} and \autoref{fig:shake_visual}).
We conjecture that this is because UCF-101 is a coarse-grained action dataset
in which the spatial (appearance) information is dominant.
As a consequence, the C3D model does not extract/need much temporal
information to perform well. %classification.
However, Jester is a fine-grained action dataset
where temporal information plays a more important role.
Therefore, in line with expectations, we find that in order to attack
the C3D model trained on the Jester dataset,
a higher extent of perturbations are required on the temporal dimension.
%the temporal information need to be perturbed more.

%A closer examination of the outputs reveals that out of all the 'sliding right' inputs misclassified, $92.8\%$ are misclassified to 'sliding two fingers right'. Both suggest that with respect to this target class, the temporal information is not perturbed much. This is because these two classes are similar and more importantly the actions depict similar (rightward) movement. On the other hand, as discussed in  \S \ref{sec:exptdesc}, there is no class which is temporally similar to 'shake hand'. Therefore to achieve misclassification, C-DUP has to create more pronounced perturbations in the temporal information as evident in the visualization.


\heading{Attack success rate:}
To showcase a comparison of the misclassification rates with respect to
the target class between the two schemes (DUP and C-DUP),
we adjust the weighting factor $\lambda$ such that the classification
accuracy with respect to non-target classes are similar.
By choosing $\lambda$ = 1.5 for DUP and 1 for C-DUP,
we are able to achieve this.
The attack success rates for the above two target sets are shown in
\autoref{fig:sliding_target} and \autoref{fig:sliding_non},
{\em and} \autoref{fig:shake_target} and \autoref{fig:shake_non}, respectively.
%{\color{red} which are fake ones right not, need to be substitute, but the trend should be similar}.
We see that with respect to $T_1=\{\text{sliding hand right}\}$,
the results are similar to what we observe with UCF101.
The attack success rates for C-DUP are a little lower than DUP when
the offset is 0. This is to be expected since DUP is tailored for this specific offset.
However, C-DUP outperforms DUP when there is a misalignment.
The average success rate for C-DUP is $85.14\%$ for the target class
and $81.03\%$ for the other (non-target) classes.
The average success rate for DUP is $52.42\%$ for the target class
and $82.36\%$ for the other (non-target) classes.

Next we consider the case with $T_2=\{\text{shaking hands} \}$.
In general, we find that both DUP and C-DUP achieve relatively
lower success rates especially with regards to the other (non-target) classes.
As discussed in  \S \ref{sec:exptdesc}, unlike in the previous case
where `sliding two fingers right' is temporally similar to `sliding hand right',
no other class is temporally similar to `shaking hand'.
Therefore it is harder to achieve misclassification.
%To capture and thus compare the misclassification rate on target class, we now  adjust the weighting factor $\lambda$ such that the classification accuracy with respect to non-target classes are similar. By choosing $\lambda = 1.5$ for DUP and 1 for C-DUP, we are able to achieve this.
\autoref{fig:shake_non} depicts the attack success rates for non-target classes.
The average success rate for non-target classes are similar
(because of the bias in $\lambda$ as discussed earlier)
and in fact slightly higher for DUP (a finer bias could make them exactly the same).
The attack success rates with the two approaches for the target class 
are shown in \autoref{fig:shake_target}.
We see that C-DUP significantly outperforms DUP in terms of misclassification
efficacy because of its robustness to temporal misalignment.
The average attack success rate for the target class with C-DUP is $79.03\%$
while for DUP it is only $57.78\%$.
Overall, our C-DUP outperforms DUP in being able to achieve a better
misclassification rate for the target class.
We believe that although stealth is affected to some extent,
it is still reasonably high.

\subsection{2D-Dual Purpose Universal Perturbations}

The visual representations of the perturbations with C-DUP show that
perturbations on all the frames are visually similar.
Thus, we ask if it is possible to add ``the same perturbation'' on every frame
and still achieve a successful attack.
In other words, will the 2D-DUP perturbation attack yield performance
similar to the C-DUP attack.

{\begin{comment}
One concern about 2D-DUP is that with same repeating perturbation, it may be hard to perturb the temporal information of the video. We guess 2D-DUP may work well on coarse-level action classification videos as in UCF-101 where appearance information is distinguished. However, it may perform not good on fine-level action classification videos like the Jester dataset where all the gestures are about hands and temporal information is more distinguished.  Therefore, the experiments on UCF101 and Jester are complementary to each other and together provide rich test cases.
}
\end{comment}

\vspace{1mm}
\subsubsection{Experimental Results on the UCF101 Dataset}~\\
\vspace{-4mm}

\heading{Visual impact of the perturbation:}
We present a sequence of original frames and its corresponding perturbed
frames in \autoref{fig:2D_CUP}.
Original frames are displayed in the first row and perturbed frames are
displayed in the second row.
We observe that the perturbation added on the frames is
quasi-imperceptible to human eyes (similar results are seen with C-DUP {\color{black} and
are presented in an appendix}).


\begin{comment}

\subsubsection{Motion information}

The intuition is that it is hard to perturb motion information with same perturbation on each frame. However, as showed in \autoref{fig:op_compare}, 2D-DUP perturbs the motion information effectively, which is surprising.

We look into further how motion information is changed. We present two other input example in \autoref{fig:motion_2d}. Combine with the example in \autoref{fig:op_compare}. We notice that it seems only two motion directions exist in the perturbed video stream, that is, the upper left motion represented by purple and the lower right motion represented by bright green. The fact that 2D perturbation has the 
ability to mask out some motion information is quite interesting.
{\color{red}{any other explanation or open question can be proposede?}}

\begin{figure*}[t!]
    \centering
    \begin{subfigure}{0.5\textwidth}
        \includegraphics[scale=.5]{images/Hula.png}
        \caption{fig:hula}
        \label{fig:base}
    \end{subfigure}
    \begin{subfigure}{0.5\textwidth}
        \includegraphics[scale=.5]{images/Boxing.png}
        \caption{fig$:$boxing}
        \label{fig:op}
    \end{subfigure}
    \caption{how motion information is changed}
    \label{fig:motion_2d}
\end{figure*}
\end{comment}


\heading{Attack success rate:}
By adding 2D-DUP on the video clip,
we achieve an attack success rate of $87.58\%$ with respect to the target class
and an attack success rate of $83.37\%$ for the non-target classes.
Recall that the average attack success rates with C-DUP were $87.52\%$ and $84.00\%$, respectively.
Thus, the performance of 2D-DUP seems to be on par with that of C-DUP on the UCF101 dataset.
This demonstrates that C3D is vulnerable even if the same 2D
perturbation generated by our approach is added on to every frame.

\vspace{1mm}
\subsubsection{Experimental Results on Jester Dataset}~\\
\vspace{-4mm}

\begin{comment}
{
\heading{Visualizing the perturbation:}  We test on two different target sets $T_1=\{\text{sliding hand right}\}$ and $T_2=\{\text{shaking hands} \}$. We visualize two perturbation generated respectively in \autoref{fig:2D_jester_t1} and \autoref{fig:2D_jester_t2} \reminder{any insight on this?}. 
}
\end{comment}

\heading{Attack success rate:}
For $T_1=\{\text{sliding hand right}\}$,
the attack success rate for the target class is $84.64\%$ and the
attack success rate for the non-target classes is $80.04\%$.
This shows that 2D-DUP is also successful on some target classes in the fine-grained,
Jester action dataset.

For the target set $T_2$, the success rate for the target class drops to $70.92\%$,
while the success rate for non-target class is $54.83\%$.
This is slightly degraded compared to the success rates achieved with C-DUP
($79.03\%$ and $57.78\%$ respectively),
but is still reasonable.
This degradation is due to more significant temporal changes in this case
(unlike in the case of $T_1$) and a single 2D perturbation is
less effective in manipulating these changes.
In contrast, because the perturbations evolve with C-DUP,
they are much more effective in achieving the misclassification of the target class.

\begin{comment}
{
The reason that the success rates are low may be as discussed in \S \ref{sec:exptdesc} that there is no class temporally similar to 'shakingshaking hand'. Therefore, we can say that the attack success rate of 2D-DUP is limited in the scenario where perturbation in appearance information is not enough to achieve attack and in this case, the proposed C-DUP is more suitable.
}
\end{comment}





==> CCS-Sasha 2/introduction.tex <==
\section{Introduction}



%This para is about motivating what is the problem we are working on and why is it important?
%larger context, why problem is of interest and importance to larger community
%--motivate the problem with the importance of video action recognition -- Important area of research in computer vision, as it is employed in automated detection of suspicious activities in surveillance or for developing autonomous driving car.

%Small change in input can cause large changes in output -> perturbations

Deep Neural Networks (DNN) have found an increasing role in 
real world applications for the purposes of real-time video classification.
Examples of such applications include video surveillance~\cite{sultani2018real},
self driving cars \cite{kataoka2018temporal}, health-care~\cite{umboocv2016case}, etc.
To elaborate, video surveillance systems capable of automated detection of undesired human
behaviors (e.g., violence) can trigger alarms and drastically reduce information workloads on human operators.
Without the assistance of DNN-based classifiers,
human operators will need to simultaneously view and assess footage from a large number of video sensors.
This can be a difficult and exhausting task,
and comes with the risk of missing behaviors of interest and slowing down decision cycles.
In self-driving cars, {video classification} has been used to
understand pedestrian actions and make navigation decisions \cite{kataoka2018temporal}.
Real-time video classification systems have also been deployed for automatic
``fall detection'' in elderly care facilities~\cite{umboocv2016case},
and abnormal detection around automated teller machines~\cite{tripathi2016real}.
All of these applications directly relate to the physical security or safety of people and property.
Thus, stealthy attacks on such real-time {video classification} systems are
likely to cause unnoticed pecuniary loss and compromise personal safety.
%Hence it is important to analyze and understand the vulnerability of such systems to adversarial attacks.  

%What is the specific problem we are considering in this paper. Here we establish specific context and background
%What has previous researchers done, and how these systems are vulnerable

Recent studies have shown that virtually all DNN-based systems are vulnerable to
well-designed adversarial inputs~\cite{moosavi2017universal,moosavi2016deepfool,
sharif2016accessorize, goodfellow2014generative,szegedy2013intriguing},
which are also referred to as \emph{adversarial examples}.
Szegedy \etal \cite{szegedy2013intriguing} showed that adversarial perturbations
that are hardly perceptible to humans can cause misclassification in DNN-based image classifiers.
Goodfellow \etal \cite{goodfellow2014explaining} analyzed the potency of
realizing adversarial samples in the physical world.
Moosavi \etal \cite{moosavi2017universal} and Mopuri \etal \cite{mopuri2017nag} introduced
the concept of ``image-agnostic'' perturbations.
As such, the high level question that we try to answer in this paper is
``Is it possible to launch stealthy attacks against DNN-based real-time
video classification systems, and if so how?''

% all of these efforts focus on adding adversarial perturbations to images.
% To the best of our knowledge, there is no work investigating whether video systems
% are susceptible to the adversarial examples.

%In this paragraph we summarize what the main contributions of our paper are given the context we have established.
Attacking a video classifier is more complex than attacking an image classifier,
because of the presence of the temporal dimension in addition to
the spatial dimensions present in 2D images.
Specifically, attacking a real-time video classifier poses additional challenges.
% To elaborate, there are multiple challenges for an attacker,
% with regards to generating perturbations to attack video classification systems.
\textit{First}, because the classification is performed in real-time,
the corresponding perturbations also need to be generated on-the-fly
with the same frame rate which is extremely computationally intensive.
\textit{Second}, to make the attack stealthy,
attackers would want to add perturbations on the video {in} such a way that
they will only cause misclassification for the targeted (possibly malicious) actions,
while keep the classification of other actions unaffected.
In a real-time video stream, since the activities change across time,
it is hard to identify online and in one-shot \cite{fanello2013one},
the target frames on which to add perturbations.
\textit{Third}, video classifiers use video clips (a set of frames)
as inputs \cite{fanello2013one,tripathi2016real}.
As video is captured, it is broken up
into clips and each clip is fed to the classifier.
As a result, even if attackers are aware of the length of each clip
(a hyper-parameter of the classifier),
it is hard to predict {\em when} each clip begins and ends.
Therefore, if they generate perturbations for a clip using traditional
methods (e.g., gradient descent), the perturbations might not work because
they are not aligned with the real clip the classifier is using
(Please see~\autoref{fig:sliding_window} and the associated discussion for more details).
%the classifier considers a temporally staggered version of that clip.

\begin{comment}
{
``how the video classification system chooses input clips'' i.e.,
%the starting point of the input clip fed to the video classification system.
it does not know
the \reminder{consecutive} sequence of frames belonging to the clip input to the classifier. 
This is problematic because the perturbations that are to be added (if generated in traditional
ways) will  
depend on \reminder{its location}
%the sequence of frames 
in the input clip.} 
}
\end{comment}


%-- real-time; Identify frames to perturb; Input boundary is not clear (where we talk about the starting point)
%we can add perturbations on all the frames, but this can change the classification results for classes other than the target class. So we need to apply this only on targeted frames, which is difficult to identify, and hence we need dual purpose perturbations which applies perturbations on all frames but still do not affect the classes other than the targetd ones. 

In this paper, our first objective is to investigate how to generate
adversarial perturbations against real-time video classification
systems by overcoming the above challenges.
We resolve the first (real-time) challenge by using {\em universal perturbations}~\cite{moosavi2017universal}.
Universal perturbations allow us to affect the classification results
using a (single) set of perturbations generated off-line.
Because they work on unseen inputs they preclude the need for intensive on-line
computations to generate perturbations for every incoming video clip.
To generate such universal perturbations, we leverage the generative
adversarial network (GAN) \cite{goodfellow2014generative} architecture.
% \reminder{,however, with the dicriminator pretrained}.
%{\color{blue}We choose {generative models} over iterative models \cite{goodfellow2014explaining,kurakin2016adversarial,carlini2017towards} because generative model is more suitable for generate things of desired features.}
%we leverage the generative adversarial network (GAN) \cite{goodfellow2014generative} architecture.
% \reminder{,however, with the dicriminator pretrained}.
%We choose {generative models} over iterative model
%because

%These perturbations can be added to the incoming feed directly.

However, adding universal perturbations on all the frames of the video can cause
the misclassification of all the actions in the video stream.
This may expose the attack as the results may not make sense (e.g., many people performing rare actions).
To make the attack stealthy,
%the attacker will have to add the perturbations such that only the targeted classes in the videos are misclassified. Towards this,
we introduce the novel concept of \textit{dual purpose universal perturbations},
which we define as universal perturbations which only cause the misclassification for
inputs belonging to the target class,
while minimize, or ideally, have no effect on the classification results
for inputs belonging to the other classes.

\begin{comment}
{
\reminder{ A good generation of dual purpose perturbations for \textit{video clips} does not guarantee the attack for \textit{video stream}}
% rate in videois not straightforward 
because (as shown in our experiments) such perturbations \reminder{may have mismatch issue on how the system chooses the input clips.}
%are dependent on ``the set of frames'' {\color{red} used as training} to generate them.} 
there might be a mismatch in terms of the clip boundaries
conceived by the attacker and that considered by the classifier.
Stated otherwise, the location of a frame in an input clip used for classification could be different
from what it was in the training clip used to determine the perturbation.
}
\end{comment}

Dual purpose perturbations by themselves do not provide high success rates
in terms of misclassification because of challenge three, which is that the mis-alignment of
the boundaries of perturbations with respect to the real clip boundaries (input to the classifier)
significantly affects the misclassification success rates.
%
To solve this problem, we introduce a new type of perturbation that
we call the \textit{Circular Universal Dual Purpose Perturbations (C-DUP)}.
The C-DUP is a 3D perturbation (i.e., a perturbation clip composed of a sequence of frames),
which is a valid perturbation on a video regardless of {the start and end of each clip}.
In other words, it works on all cyclic permutations of frames in a clip.
%{\color{black} where it is added} i.e., it is agnostic to the sequence of frames in the input clip.
To generate the C-DUP, we make significant changes to the baseline GAN architecture.
In particular, we add a new unit to generate circular perturbations,
that is placed between the generator and the discriminator (as discussed later).
We demonstrate that the C-DUP {\color{black} is very {stable and effective}
in {achieving real-time stealthy attacks on video classification systems}.
%causing the misclassification of only the targeted actions in the input videos}.

After demonstrating the feasibility of stealthy attacks against real-time
video classification systems, our second objective is to investigate the effect
of the temporal dimension.
In particular, we investigate the feasibility of attacking the classification
systems using a simple and light 2D perturbation
which is applied across all the frames of a video.
% causes the misclassification as expected.
By tweaking our generative model, we are able to generate such perturbations
which we name as \textit{2D Dual Purpose Universal Perturbations (2D-DUP)}.
These perturbations work well on a sub-set of videos, but not all.
We will discuss the reasons for these 2D attacks in \S~\ref{sec:2D}.

\medskip
\noindent \textbf{Our Contributions:}
In brief, our contributions in this paper are:

%specify little bit on our experiments here.
\squishlist
	%\item We provide a comprehensive analysis on why the way perturbations crafted for
	%the image domain do not directly extend to the video domain.
	\item We provide a comprehensive analysis on the challenges in crafting
	adversarial perturbations for real-time video classifiers.
	We empirically identify what we call the boundary effect phenomenon in
	generating adversarial perturbations against video (see~\S~\ref{sec:temporal}).

	% demonstrate stealth attacks against real-time video classification systems
	\item We design and develop a generative framework to craft two types of
	stealthy adversarial perturbations against real-time video classifiers, viz.,
	circular dual purpose universal perturbation (C-DUP)
	and 2D dual purpose universal perturbation (2D-DUP).
	These perturbations are agnostic to (a) the video captured (universal) and
	(b) the temporal sequence of frames in the clips input to the video classification system
	(resistance to cyclic permutations of frames in a clip).

	%the sequence of frames used by the classifier for inference  \autoref{sec:solution}).
	\item We demonstrate the potency of our adversarial perturbations using two different video datasets.
	%each depicting a different type of activity.
	In particular, the UCF101 dataset captures coarse-grained activities
	(human actions such as applying eye makeup, bowling, drumming) \cite{soomro2012ucf101}.
	The Jester dataset captures fine-grained activities
	(hand gestures such as sliding hand left, sliding hand right, turning hand clockwise, turning hand counterclockwise) \cite{jester2016}.
	We are able to launch stealthy attacks on both datasets %misclassify the target class
	with over a 80 \% misclassification rate,
	while ensuring that the other classes are correctly classified with {relatively high accuracy}.
	%over 85 \% accuracy. %{\color{red} Provide citations for datasets}
\squishend

\begin{comment}
{
	\item As a specific use case of our methodology, we {\color{blue}generate perturbations for videos comment: not a good way to put it, because again, easily to get perturbation for DNNs}from two standard datasets, UCF101 and Jester . We empirically show the success of the proposed perturbations in misclassifying the targeted actions \textbf{while not effecting the other classification much} (see \autoref{sec:evaluation}). 
\end{enumerate}

%What have been done, and what we are doing. 

In this study we propose two different types of perturbations to attack video classification systems. To validate the potential of our perturbations in misclassifying videos, we run experiments on two standard datasets UCF101 and Jester. Jester has variety of motion focused dataset, while UCF101 has diverse activities, so these two datasets provide us rich environment to test our attack models. On UCF101 dataset, we show that the addition of circular dual purpose universal perturbations could successfully fool the classification system with the accuracy of 85\%. Similarly, on Jester dataset, we observe the attack success rate of 85\%. Also, with 2D we validate this perturbation successfully misclassifies the videos in Jester dataset with the success rate of ...... 
}
\end{comment}


==> CCS-Sasha 2/real2.tex <==
\section{Generating perturbations for real-time video stream}
\label{sec:realtime}
\begin{figure}[t]
	\centering
	\begin{subfigure}{0.5\textwidth}
		\includegraphics[scale=.22]{images/GAN_arc.png}
		\vspace{-15mm}
		\subcaption{GAN Architecture}
		\vspace{5mm}
		\label{fig:gan_arc}    
	\end{subfigure}
	\begin{subfigure}{0.5\textwidth}
		\includegraphics[scale=.20]{images/Our_arc.png}
		\subcaption{Our Architecture}
		\label{fig:our_arc}   
	\end{subfigure}
	\caption{This figure compares our architecture with traditional GAN architectures. Our architecture is different fromtraditional GAN in the following aspects: 1) The discriminator is a pre-trained classifier we attack, whose goal is to classify videos, and not to distinguish between the natural and synthesized inputs; 2) The generator generates perturbations, and not direct inputs to the discriminator, and the perturbed training inputs are fed to discriminator; 3) The learning objective is to let the discriminator misclassify the perturbed inputs.}
	\label{fig:arc}
\end{figure}

From the adversary's perspective, we first consider
the challenge of attacking a real-time video stream.
% that a video classification system takes
In brief, when attacking an image classification system, the attackers usually take the 
following approach. First, they obtain the {\em target} image that is to be attacked with its true label. 
Next, they formulate a problem wherein they try to compute the ``minimum'' noise that is to be
added in order to cause a mis-classification of the target.
The formulation takes into account the function of the classifier, the input image, and its true label. 
In contrast, in the context of real-time video classification, the video is not available to the attackers a priori.
Thus, they will need to create perturbations that can effectively perturb an incoming video stream,
whenever a {\em target class} is present.

Our approach is to compute the perturbations offline and apply them online.
% in a real-time video classification system.
Since we cannot predict what is captured in the video, we need perturbations
which work with unseen inputs. A type of perturbations that satisfies this requirement
is called the Universal Perturbation (UP), which has been studied in
the context of generating adversarial samples against image classification
systems~\cite{mopuri2017nag,moosavi2017universal}.
In particular, Mopuri \etal, %, as discussed earlier in \S~\ref{sec:nag},
have developed a generative model that learns the space of universal perturbations for images
using a GAN-like architecture.
%, they train a discriminator, and the generator learns how to synthesize \reminder{perturbation by %inputs to conform with the space covered by the training set. Their architecture is depicted in Fig.~\ref{fig:gan_arc}. 

Inspired by this work, we develop a similar architecture,
but make modifications to suit our objective.
Our goal is to generate adversarial perturbations that fool the
discriminator instead of exploring the space for diverse UPs.
In addition, we retrofit the architecture to handle video inputs.
Our architecture is depicted in \autoref{fig:our_arc}.
It consists of three main components:
1) a 3D generator which generates universal perturbations;
2) a post-processor, which for now does not do anything but is needed
to solve other challenges described in subsequent sections; and
3) a pre-trained discriminator for video classification,
e.g., the C3D model described in \S~\ref{sec:c3d}.
Note that unlike in traditional GANs
wherein the generator and the discriminator are trained together,
we only train the generator to generate universal perturbations to
fool a fixed type of discriminator.

The 3D generator in our model %used to generate universal perturbations in our study is similar to the one employed by Mopuri \etal \cite{mopuri2017nag}, except that our generator
is configured to use 3D deconvolution layers and provide 3D outputs as shown in \autoref{fig:arc_roll}.
Specifically, it generates a clip of perturbations,
whose size is equal to the size of the video clips taken as input by the C3D classifier.
%The architecture of the generator and the hyper-parameter are shown in \autoref{fig:arc_roll}.
To generate universal perturbations, the generator first takes a noise vector $z$ from a latent space.
Next, It maps $z$ to a perturbation clip $p$, such that, $G(z)=p$.
It then adds the perturbations on a training clip $x$ to obtain the perturbed clip $x+p$.
Let $c(x)$ be the true label of $x$.
This perturbed clip is then input to the
C3D model which outputs the score vector $Q(x+p)$ (for the perturbed clip).
The classification should ensure that the highest score corresponds to
the true class
($c(x)$ for input $x$) %the class that $x$ belongs to
in the benign setting.
Thus, the attacker seeks to generate a $p$ such that the C3D classifier outputs
a low score to the $c(x)$th element in $Q$ vector (denoted as $Q_{c(x)}$) for $x+p$.
In other words, this means that after applying the perturbation,
the probability of mapping $x$ to class $c(x)$ is lower than the
probability that it is mapped to a different class
(i.e., the input is not correctly recognized).

We seek to make this perturbation clip $p$ ``a universal perturbation'',
i.e., adding $p$ to any input clip belonging to the target class
would cause misclassification.
This means that we seek to minimize the sum of the cross-entropy loss
over all the training data as per \autoref{equ:cross_entr}.
Note that the lower the cross-entropy loss,
the higher the divergence of the predicted probability from the true label~\cite{huang2017stacked}.

\begin{equation}
\underset{G}{\text{minimize}}\quad \sum_{x\in X}{-\log[1-Q_{c(x)}(x+G(z)]}
\label{equ:cross_entr}
\end{equation}

When the generator is being trained, for each training sample,
it obtains feedback from the discriminator and adjusts its parameters % so as to try
to cause the discriminator to misclassify that sample.
It tries to find a perturbation that works for every sample
from the distribution space known to the discriminator.
At the end of this phase, the attacker will have a generator
that outputs universal perturbations which can cause the misclassification on any
incoming input sample from the same distribution (as that of the training set).
However, as discussed next, just applying the universal perturbations alone
will not be sufficient to carry out a successful attack.
In particular, the attack can cause unintended clips to be misclassified as well,
which could compromise our stealth requirement as discussed next in \S \ref{sec:perturbframe}.
%weight, and bias are the parameter which the generator adjusts after getting, feedback is the Q(c) score. 
\begin{comment}
 In addition, to dealing with video classifier, we use a 3D generator instead of 2D generator in \cite{mopuri2017nag} We extend this framework to generate perturbations for videos. In particular, we replace the discriminator with a video classification classifier, and develop a 3D universal perturbation generator. We depict our framework in \autoref{fig:arc}.

Let us denote the clean input clip as $x$, and the perturbation clip as $p$. We denote the output vector of the softmax layer of the discriminator as $Q(x)$, and {\color{blue}the true label of the input as $c(x)$. 
Ideally, a good discriminator should output the largest probability at $Q[c(x)]$ (denoted $Q_{c(x)}$
for ease of exposition), i.e.,
the input is correctly classified. 
We formulate the loss function formulate the loss function for generating the UP as follows: 

As discussed in \autoref{sec:boundary}, the UPs generated with this loss easily come into boundary problem when testing, which causes the attack success rate to be low when the chosen input clips dis-matches the added perturbation clips. 
{\color{red} Guys: We need to give intuition as to why this is reasonable.}
\end{comment}



==> CCS-Sasha 2/rel.tex <==
\section{Related Work}
%{\color{red}{show the common methods to fool image classifier is to use "back propagate kind of methods', which need computation for each new seen input.}}
%{\color{red} need to specific the GAN-like architecture of NAG, basically explain how NAG generate perturbations}

There is quite a bit of work \cite{biggio2013evasion,biggio2014pattern,huang2011adversarial} on
investigating the vulnerability of machine learning systems to adversarial inputs. 
Researchers have shown that generally, small magnitude perturbations added to input samples, 
change the predictions made by machine learning models. 
Most efforts, however, do not consider real-time temporally varying inputs such as video.
Unlike these efforts, our study is focused on the generation of adversarial perturbations to fool DNN based real-time video action recognition systems. 


The threat of adversarial samples to deep-learning systems has also received considerable attention recently. There are several papers in the literature (e.g., \cite{moosavi2017universal,moosavi2016deepfool,sharif2016accessorize, goodfellow2014generative,goodfellow2014explaining}) that have shown that 
the state-of-the-art DNN based learning systems are also vulnerable to well-designed adversarial 
perturbations \cite{szegedy2013intriguing}. Szegedy \etal show that the addition of 
hardly perceptible perturbation on an image, can cause a neural network to misclassify the image. 
Goodfellow \etal \cite{goodfellow2014explaining} analyze the potency of adversarial samples available in the physical world, in terms of fooling neural networks. 
Moosavi-Dezfooli \etal \cite{moosavi2017universal, moosavi2016deepfool,mopuri2017fast} make a significant
contribution by generating image-agnostic perturbations, which they call universal adversarial perturbations. 
These perturbations can cause all natural images belonging to target classes to be misclassified 
with high probability.  

%To explore the space of the distribution of universal adversarial perturbations, 
%Mopuri \etal \cite{mopuri2017nag} introduce a generative approach based on GANs. 

GANs or generative adversarial networks have been employed by Goodfellow \etal \cite{goodfellow2014generative} and Radford \etal \cite{radford2015unsupervised} in generating natural images. 
Mopuri \etal \cite{mopuri2017nag} extend a GAN architecture to train a generator to model 
universal perturbations for images. Their objective was to explore the space of
the distribution of universal adversarial perturbations in the image space. 
We significantly extend the generative framework introduced by Mopuri \etal \cite{mopuri2017nag}. 
In addition, unlike their work which focused on generating adversarial perturbations for images, our study focuses on the generation of effective perturbations to attack videos.

The feasibility of adversarial attacks against other types
of learning systems including face-recognition systems \cite{sharif2016accessorize,mccoyd2016spoofing,sharif2017adversarial}, 
voice recognition systems \cite{carlini2016hidden} and malware classification systems \cite{grosse2016adversarial} has been studied. However, these studies do not account for the unique input characteristics 
that are present in real-time video activity recognition systems.




==> CCS-Sasha 2/stealth2.tex <==
\section{making perturbations stealthy}
\label{sec:perturbframe}

Blindly adding universal perturbations will affect the classification of
clips belonging to other non-targeted classes. %other than the target class.
This may raise alarms, especially if many of such misclassifications are mapped on to rare actions.
Thus, while causing the target class to be misclassified,
the impact on the other classes must be imperceptible.
This problem can be easily solved when dealing
with image recognition systems since images are self-contained entities,
i.e., perturbations can be selectively added on target images only.
%and while no perturbation is added on to other images (not capturing the target).
However, video inputs change temporally and an action captured in a set of
composite frames may differ from that in the subsequent frames.
It is thus hard to a priori identify (choose) the frames relating to the target class,
and add perturbations specifically on them.
For example, consider a case with surveillance in a grocery store.
If attackers seek to misclassify an action related to shoplifting and
cause this action to go undetected,
they do not have a priori knowledge about when this action will be captured.
And adding universal perturbations blindly could cause mis-classifications of other actions (e.g.,
other benign customer actions may be mapped onto shoplifting actions thus triggering alarms).

Since it is hard (or even impossible) to a priori identify the frame(s)
that capture the intended actions and choose them for perturbation,
the attackers need to add perturbations on each frame.
However, to make these perturbations furtive,
they need to ensure that the perturbations added only mis-classifies
the target class while causing other (non-targeted) classes to be classified correctly.
We name this unique kind of universal perturbations as  ``Dual-Purpose Universal Perturbations''
or DUP for short.

In order to realize DUPs, we have to guarantee that for the input clip $x_t$,
if it belongs to the target class (denote the set of inputs from target class as $T$),
the C3D classifier returns a low score with respect to the correct class $c(x_t)$,
i.e., $Q_{c(x_t)}$.
For input clips $x_s$ that belongs to other (non-target) classes
(denote the set of inputs from non-target classes as $S$, thus, $S=X-T$),
the model returns high scores with regards to their correct mappings ($Q_{c(x_s)}$).
%{\color{red} Here using the same notation for both intended class and unintended classes
%is confusing. Can we use different variables to represent?}
%$Q_c$ refers to the position of the class in the score vector.
To cause the generator to output DUPs, we refine the optimization problem in \autoref{equ:cross_entr}
%. Specifically, we \reminder{divide the optimization loss into two parts}
as shown in \autoref{equ:dual}:

	\begin{equation}
	\begin{aligned}
	\underset{G}{\text{minimize}} \quad & \lambda\times \sum_{x_t\in T}{-\log[1-Q_{c(x_t)}(x_t+G(z))]}\\
	                              &+\sum_{x_s\in S}{-\log[Q_{c(x_s)}(x_s+G(z))]}
	\end{aligned}
	\label{equ:dual}
	\end{equation}

	%We denote the set of inputs belong to target class(es) as $T$, and the weight between these two objectives as $\lambda$, then the fooling loss can be formulated as follow.

The first term in the equation again relates to minimizing the cross-entropy of the target class,
while the second term maximizes the cross-entropy relating to each of the other classes.
The parameter $\lambda$ is the weight applied with regards to the misclassification of the target class.
For attacks where stealth is more important, we may use a smaller $\lambda$ to guarantee that the
emphasis on the
misclassification probability of the target class is reduced while
the classification of the non-target classes are affected to the least extent possible.

	%\reminder{Next, we need to explain the loss function, and differentiate it with the loss function used in universal perturbation}


==> CCS-Sasha 2/temp2.tex <==
\section{The time machine: handling the temporal dimension}
\label{sec:temporal}

The final challenge that the attackers will need to address in order to effectively generate
adversarial perturbations against real-time video classification systems
is to handle the temporal structure that exists across the frames in a video.
In this section, we first discuss why directly applying existing methods
that target images to generate perturbations against video streams do not work.
Subsequently, we propose a new set of perturbations that overcome this challenge.

\begin{figure}%[t]
	\centering
	\begin{subfigure}{0.5\textwidth}
		\includegraphics[scale=.4]{images/explain_mismatch.png}
		\subcaption{This figure depicts a scenario where there is a mismatch between the clip an attacker views to generate a perturbation, and the clip a classifier views for classification.}
		\label{fig:mismatch}
	\end{subfigure}

	\vspace{0.02\textwidth}
	\begin{subfigure}{0.5\textwidth}
		\includegraphics[scale=.4]{images/explain_stride_overlap.png}
		\subcaption{This figure displays a scenario where the stride of the sliding window is smaller than the size of a clip. In such a case, the attacker will not know what perturbation to use on a frame, as the frame can be selected in multiple input clips
used in classification.}
		\label{fig:stride_overlap}
	\end{subfigure}
	\caption{The sliding window used to capture clips that are input to the video classification system}
	\label{fig:sliding_window}
\end{figure}
\subsection{The boundary effect
%clips used for perturbation generation would be different from the clips used for testing.
}

The input to the video classifier is a clip of a sequence of frames.
As discussed earlier, given an input clip,
it is possible to generate perturbations for each frame in that clip.
However, the attacker cannot a priori determine the {\em clip boundaries} used
by the video classifier.
In particular, as discussed in \S~\ref{sec:var}, there are
three hyper-parameters that are associated with a sliding window of a video classifier.
They are the {\em window size}, the {\em stride} and the {\em starting position} of the clip.
All three parameters affect the effectiveness of the perturbations.
While the first two parameters are known to a white-box attacker,
the last parameter is an artifact of when the video clip is captured and input to the
classifier and cannot be known a priori.

The perturbation that is to be added to a frame depends on the relative
location of the frame within the clip.
In other words, if the location of the frame changes because of a temporally staggered clip,
the perturbation needs to adjusted accordingly.
Thus at a high level, the boundaries of the clips used by the classifier
will have an effect on the perturbations that need to be generated.
We refer to this phenomenon as the boundary effect.
To formalize the problem, let us suppose that there is a video stream represented by
$\{ ...,f_{i-2}, f_{i-1}, f_i,
f_{i+1},f_{i+2}, ...\}$ where each $f_j$ represents a frame.
The perturbation on $f_i$ that is generated based on
the clip [$f_{i}, f_{i+1}, \cdots, f_{i+w-1}$] to achieve misclassification of
a target action, will be different from the one generated based on the
temporally staggered clip $[f_{i-1}, f_{i}, f_{i+1} \cdots, f_{i+w-2}]$ to
achieve the same purpose.

To exemplify this problem, we consider using the traditional methods
to attack C3D model. In particular, we use the API from the CleverHans
repository \cite{papernot2016cleverhans} to generate video perturbations.
Note that, the perturbations generated by CleverHans are neither universal nor dual-purpose;
they simply generate a specific perturbation given a specific input clip.
We use the basic iteration methods with default parameters.
Our approach is as follows.
We consider all the videos in the UCF-101 testing set.
We consider different boundaries for the clips in the videos
(temporally staggered versions of the clips) and use the Python libraries
from CleverHans to generate perturbations for each staggered version.
Note that the sliding window size for C3D is 16 and thus, there are 16 staggered versions.
We choose a candidate frame, and compute the correlations between the perturbations added in the
different staggered versions. Specifically, the perturbations are tensors and the normalized correlation
between two perturbations is the inner product of the unit-normalized tensors representing the perturbations.

We represent the average normalized correlations in the perturbations (computed across all videos and all frames)
for different offsets (i.e., the difference in the location of the
candidate frame in the two staggered clips) 
in the matrix shown in \autoref{fig:corre}.
The row index and the column index represent the location of the frames
in the two staggered clips.
For example, the entry corresponding to $\{7,7\}$ represents
the case where the frame considered was the $7^{th}$ frame in the two clips.
In this case, clearly the correlation is 1.00.
However, we see that the correlations are much lower if the
positions of the same frame in the two clips are different.
As an example, consider the entry $\{5, 9\}$:
its average normalized correlation is 0.39,
which indicates that the perturbations that CleverHans adds in the
two cases are quite different.

\begin{comment}
{
We use the existing popular perturbation generation method basic iteration~\cite{kurakin2016adversarial}
{\color{blue} may get results from other existing attack methods if time allowed}
to showcase the boundary effect problem.
We use the API from CleverHands \cite{papernot2016cleverhans}, an Python libary to generate perturbations for all the videos from UCF-101 testing set based on C3D model (see \autoref{sec:c3d}). The maximum perturbation on each pixel is set to be 10 (the image is represent in [0,255]). The step size for each attack iteration is set to be 1 and the number of attack iterations is set to be 14. We set the attack to be untargeted attack, which means, we want the clips to be misclassified to any label.

We then test the correlation between these different perturbations on the same frames. Averaged correlation matrix is shown in \autoref{fig:corre}. Both the row and the column represents the location of the frame and the value showed in row $r$ and column $c$ means the normalized correlation between the perturbation generated when it is the $r$th frame and the $c$th frame in the input clips. The result show that the perturbations on the same frames are different quantitively.
}
\end{comment}

\begin{figure}[!ht]
	\centering
	\includegraphics[scale=0.33]{images/correlation_untarg_10.png}
	\caption{The average normalized correlation matrix computed with perturbations generated using 
the basic iteration API from CleverHans. Both row and column represent the location of frame in clips and the value represents the correlation between perturbations on the same frames but generated when that frame located in different positions in the two temporally staggered clips.}
	\label{fig:corre}
\end{figure}

In \autoref{fig:mag_per}, we show
the average magnitude of perturbations added (over all frames and all videos),
when the target frame is at different locations within a clip.
The abscissa depicts the frame position,
and the ordinate represents the magnitude of the average perturbation.
We observe that the magnitude of the perturbation on the first and last
few frames are larger than those in the middle.
We conjecture this is because the difference in perturbation between
consecutive frame locations are similar
(because the clips with small temporal offsets are similar);
but as the frame location differs by a lot, the perturbation
difference will again go up (clips with larger offsets will be more diverse).
%This means, when the same frame is located at the start or the end part of the input clip, it gets larger distortion.

\begin{figure}[!ht]
	\centering
	\includegraphics[scale=0.25]{images/mag_per_10_untarget.png}
	\caption{Magnitude of perturbation on each frame: The x axis is the frame position, and the y axis is the magnitude of average perturbation on the frame. }
	\label{fig:mag_per}
\end{figure}



We further showcase the impact of the boundary effect by measuring
the degradation in attack efficacy due to mismatches between
the anticipated start point when the perturbation is generated
and the actual start point when classifying the clip
(as shown in \autoref{fig:mismatch}).
%In other words, we assume that the frame is always at the beginning of the clip, and examine the mis-match in attack success rate if it is located elsewhere in the clip.
\autoref{fig:dismatch_1} depicts the results.
The abscissa is the offset between the clip considered for
perturbation generation and the clip used in classification.
We can see that as the distance between the two start points increases,
the attack success rate initially degrades but
increases again as the clip now becomes similar to the subsequent clip.
%and as a consequence, the success rate climbs up again
For example, if the offset is 15, the clip chosen %\reminder{is very similar to the subsequent clip).}
is almost identical to the subsequent clip.

The boundary effect is also experienced when the stride used by the
classifier is smaller than the clip size.
In brief, stride refers to the extent to which the receiver's sliding
window advances when considering consecutive clips during classification.
If the stride is equal to the clip size,
there is no overlap between the clips that are considered as inputs for classification.
On the other hand, if the stride is smaller than the size of the clip,
which is often the case \cite{tran2015learning,carreira2017quo,fanello2013one,tripathi2016real},
the clips used in classification will overlap with each other
as shown in \autoref{fig:stride_overlap}.
A stride that is smaller than the clip size will cause the same problem
discussed above with respect to the temporal offset between the attackers'
anticipation of the start point and the actual start point of the classifier.
As evident from the figure, such a stride induces an offset,
and this results in the same behaviors that we showcased above.

\begin{comment}

\reminder{The impact of boundary effect happens not only when there is mismatch. Suppose the stride is smaller than the size of sliding window, some frames are overlapped by two or even more input clips. Then there comes problem how to add perturbation when there are two different perturbations generated as shown in \autoref{fig:stride_overlap}.}
}
\end{comment}
\begin{comment}
{
e the way perturbations added on the video stream mismatches the way sliding window chooses input clips. We use offset to measure the extend to which mismatch happens. The experiment result is showed in \autoref{fig:mismatch}. The x axis is the offset between the clip generating perturbation and the clip tested. The y axis is the attack success rate. The results show boundary effect harms the attack a lot if there is mismatch.
 %We measure the harm on target attack, which means, we want the clips to be misclassified to any label. The attack target is set to be the least likely class predicted by the network as suggested by \cite{kurakin2016adversarial, kurakin2016adversarial} The maxinum perturbation on each pixel is set to be 15.The result is showed in \autoref{fig:dismatch_2}. As we can see, target attack harms more from this mismatch problem.
}
\end{comment}

\begin{figure}[!ht]
	\centering
	\includegraphics[scale=0.3]{images/untarget_10_accuracy.png}
	\caption{Attack success rate when there is mismatch. The x axis is the offset between the clip generating perturbation and the clip tested. The y axis is the attack success rate.}
	\label{fig:dismatch_1}
\end{figure}

%\begin{subfigure}{0.3\textwidth}
%	\includegraphics[scale=0.35]{images/target_15_accuracy.png}
%	\caption{target attack, 15}
%	\label{fig:dismatch_2}
%\end{subfigure}

\begin{comment}
{
To conclude, perturbations on same frame are different when locating in different input clips, and this difference affects the attack success rate.


\subsubsection{Input boundaries of video stream are not deterministic}
\label{sec:boundary}

Given a real-time video stream, there is no deterministic boundary for video clips.
To recall (see \autoref{sec:var}), the input for the classifier is chosen by the sliding window. There are three parameters related to the sliding window; window size, starting position, and the stride. Any change on one of these three parameters will result in different input clip and thus different boundaries between video clips. 

Since it is hard for an attacker to know the starting position, it is hard to know in advance where the boundaries of an input clip are. To make things worse, if the stride of sliding is smaller than $w$, one frame can be located in more than one input clips and it will be challenging to deal with these conflicts as showed in \autoref{fig:stride_overlap}.

The fact that current generated perturbations have boundary effect and there is no clear boundary for video task make attack on VAR challenging.
}
\end{comment}

\begin{figure}[ht!]
	\centering
	\includegraphics[scale=.2]{images/generator_roll.png}
	\caption{This figure illustrates the Generator and Roll for generating C-DUP.
	1) The generator takes a noise vector as input, and outputs a perturbation clip with 16 frames. The output size for each layer is shown as $\text{temporal dimension} \times \text{horizontal spatial dimension} \times \text{vertical spatial dimension} \times \text{number of channels}$. 2) The roll part shifts the perturbation clip by some offset. The figure shows one example where we roll the front black frame to the back.}
	\label{fig:arc_roll}
\end{figure}
\begin{figure}
	\includegraphics[scale=.22]{images/generator_tile.png}
	\caption{This figure illustrates the Generator and Tile for generating 2D-DUP.
	1) The generator takes a noise vector as input, and outputs a single-frame perturbation. 2) The tile part constructs a perturbation clip by repeating the single-frame perturbation generated 16 times.}
	\label{fig:arc_tile}
\end{figure}


\subsection{Circular Dual-Purpose Universal Perturbation}
\label{sec:CDUP}

The above discussion shows that the boundary effect makes it especially
challenging to attack video classification systems.
To cope with this effect, we significantly extend
the DUPs proposed in \S~\ref{sec:perturbframe} to compose what we call
``Circular Dual-Purpose Universal Perturbations (C-DUP).''

Let us uppose that the size of sliding window is $w$.
Then, the DUP clip $p$ includes $w$ frames (of perturbation),
denoted by $[p_1,p_2, \cdots, p_w]$.
Since $p$ is a clip of universal perturbations,
we launch the attack by repeatedly adding perturbations on each consecutive clip consisting of
$w$ frames, in the video stream.
One can visualize that we are generating a perturbation stream which
can be represented as $[\cdots,p_{w-1}, p_w,p_1,p_2,\cdots ]$.
Now, our goal is to guarantee that the perturbation stream works
regardless of the clip boundaries chosen by the classifier.
In order to achieve this goal,
we need any {\em cyclic or circular shift} of the DUP clip to yield a valid perturbation.
In other words,
we require the perturbation clips $[p_w,p_1,\cdots,p_{w-1}]$, $[p_{w-1},p_w,p_1,\cdots,p_{w-2}]$,
and so on, all to be valid perturbations.
To formalize, we define a permutation function $Roll(p,o)$ which yields
a cyclic shift of the original DUP perturbation by an offset $o$.
In other words, when using $[p_1,p_2, \cdots, p_w]$ as input to $Roll(p,o)$,
the output is $[p_{w-o},p_{w-o+1}, \cdots p_{w}, p{1} \cdots p_{w-o-1}]$.
Now, for all values of $o \in \{0,w-1\}$,
we need $p_o=Roll(p,o)$ to be a valid perturbation clip as well.
Towards achieving this requirement, we use a post-processor unit
%(referred to earlier in \S~\ref{sec:realtime}),
which applies the roll function between the generator and the discriminator.
This post processor is captured in the complete architecture is shown in \autoref{fig:our_arc}.

The details of how the generator and the roll unit operate
in conjunction are depicted in \autoref{fig:arc_roll}.
As before, the 3D generator ($G$) takes a noise vector as input and
outputs a sequence of perturbations (as a perturbation clip).
Note that the final layer is followed by a $tanh$ non-linearity which
constrains the perturbation generated to the range [-1,1].
The last thing is to scale the output by $\xi$.
Doing so restricts the perturbation's range to $[-\xi,\xi]$.
Following the work in \cite{moosavi2017universal,mopuri2017nag},
the value of $\xi$ is chosen to be 10 towards making the perturbation quasi-imperceptible.
The roll unit then ``rolls'' (cyclically shifts)
the perturbation $p$ by an offset in $\{0,1,2,\cdots,w-1\}$.
\autoref{fig:arc_roll} depicts the process with an offset equal to 1;
the black frame is rolled to the end of the clip.
By adding the rolled perturbation clip to the training input,
we get the perturbed input.
As discussed earlier, the C3D classifier takes the perturbed input and
outputs a classification score vector.
As before, we want the true class scores to be (a) low for the targeted inputs
and (b) high for other (non-targeted) inputs.
We now modify our optimization function to incorporate the roll function as follows.

\begin{comment}
\subsubsection{Discriminator}
Same as \cite{mopuri2017nag}, the discriminator is trained before training the generator and are frozen during the training of the generator.
As presented in \autoref{sec:c3d}, C3D is the state-of-art classifier for human action recognition. Therefore C3D is used as our discriminator. 
To experiment on Jester dataset, we fine-tunde the C3D.
\end{comment}

%Therefore, the final loss function can be formulated as follow.

\begin{equation}
\begin{aligned}
\underset{G}{\text{minimize}} \quad \sum_{o=1,2\cdots w}\{\lambda\times \sum_{x_t\in T}
{-\log[1-Q_{c(x_t)}(x_t+Roll(G(z),o))]}\\
+\sum_{x_s\in S}{-\log[Q_{c(x_s)}(x_s+Roll(G(z),o))]}\}
\end{aligned}
\end{equation}

The equation is essentially the same as Equation~\ref{equ:dual},
but we consider all possible cyclic shifts of the perturbation output by the generator.
%\reminder {In practice, during training, we choose randomly offsets for the perturbations for the sake of efficiency.}


\subsection{2D Dual-Purpose Universal Perturbation}
\label{sec:2D}

We also consider a special case of C-DUP,
wherein we impose an additional constraint which is that ``the perturbations added on
all frames should be the same.''
In other words, we seek to add a single 2D perturbation on each frame
which can be seen as a special case of C-DUP with $p_1 = p_2 = \cdots = p_w$.
We call this kind of DUP as 2D-DUP.
2D-DUP allows us to examine the effect of the temporal dimension in generating
adversarial perturbations on video inputs.

The generator in this case will output a single-frame perturbation
instead of a sequence of perturbation frames as shown in \autoref{fig:arc_tile}.
This is a stronger constraint than the circular constraint,
which may cause the attack success rate to decrease (note that the cyclic property still holds).
However, with this constraint, the perturbation generated is
much simpler and easier to use.

We denote the above 2D perturbation as $p_{2d}$.
The perturbation clip is then generated by simply creating copies of
the perturbation and {\em tiling} them to compose a clip.
The 2D-DUP clip is now $p_{tile} = [p_{2d}, p_{2d}, \cdots, p_{2d}]$
(see \autoref{fig:arc_tile}).
Thus, given that the attack objective is the same as before,
we simply replace the $Roll(p,o)$ function with a $Tile$ function
and our formulation now becomes:

\begin{equation}
\begin{aligned}
\underset{G_{2D}}{\text{minimize}}\quad \lambda\times \sum_{x_t\in T}{-log[1-Q_{c(x_t)}(x_t+Tile(G_{2D}(z)))]}\\
+\sum_{x_s\in S}{-log[Q_{c(x_s)}(x_s+Tile(G_{2D}(z)))]}
\end{aligned}
\end{equation}




==> CCS-Sasha 2/temporaldimension_shasha.tex <==
\section{The time machine: handling the temporal dimension}
\label{sec:temporal}
In this section, we discuss why directly applying existing methods to generate perturbation for video stream do not work, and propose our novel perturbations to solve the problem.
\begin{figure}%[t]
	\centering
	\begin{subfigure}{0.5\textwidth}
		\includegraphics[scale=.4]{images/explain_mismatch.png}
		\subcaption{mismatch}
		\label{fig:mismatch}    
	\end{subfigure}
	\begin{subfigure}{0.5\textwidth}
		\includegraphics[scale=.4]{images/explain_stride_overlap.png}
		\subcaption{overlap}
		\label{fig:stride_overlap}   
	\end{subfigure}
	\caption{sliding window}
	\label{fig:sliding_window}
\end{figure}
\subsection{Motivation}

\subsubsection{Boundary effect existing in perturbations}
Perturbation is generated by optimising the input of the DNNs toward misclassication. Since the input for the video classifier is a sequence of frames (we mention it as clip afterward), the perturbation is generated driven by input clips.
However, when a frame is located in different clip, the perturbation generated for it are different. This means the boundaries of the clips will have an effect on the perturbations generated. We name this as boundary problem. To elaborate, suppose a video stream $\{ ...,f_{i-2}, f_{i-1}, f_i,
f_{i+1},f_{i+2}, ...\}$, the perturbation on $f_i$ generating by choosing clip [$f_{i}, f_{i+1}, \cdots, f_{i+w-1}$] is different from the one generated by clip [$[_{i-1}, f_{i}, f_{i+1} \cdots, f_{i+w-2}]$].
Therefore, whether the boundary of input clips chosen between $f_{i-1}$ and $f_{i}$ or between $f_{i-2}$ and $f_{i-1}$ influences the perturbation on $f_i$, and also on the other frames.

We use the existing popular perturbation generation method basic iteration~\cite{kurakin2016adversarial}
%four currently existing popular perturbation generation methods namely, fast gradient~\cite{goodfellow2014explaining}, basic iteration~\cite{kurakin2016adversarial}, CarliniWagnerL2~\cite{carlini2017towards}, and saliency map \cite{papernot2016limitations} 
{\color{blue} may get results from other existing attack methods if time allowed}
to showcase the boundary effect problem.
We use the API from CleverHands \cite{papernot2016cleverhans}, an Python libary to generate perturbations for all the videos from UCF-101 testing set based on C3D model (see \autoref{sec:c3d}). The maximum perturbation on each pixel is set to be 10 (the image is represent in [0,255]). The step size for each attack iteration is set to be 1 and the number of attack iterations is set to be 14. We set the attack to be untargeted attack, which means, we want the clips to be misclassified to any label.

We then test the correlation between these different perturbations on the same frames. Averaged correlation matrix is shown in \autoref{fig:corre}. Both the row and the column represents the location of the frame and the value showed in row $r$ and column $c$ means the normalized correlation between the perturbation generated when it is the $r$th frame and the $c$th frame in the input clips. The result show that the perturbations on the same frames are different quantitively.  

\begin{figure}[!ht]
	\centering
	\includegraphics[scale=0.3]{images/correlation_untarg_10.png}
	\caption{correlation matrix,to be explained further}
	\label{fig:corre}
\end{figure}

We measure the average magnitude of perturbations on different locations as shown in \autoref{fig:mag_per}. The x axis is the frame position, and the y axis is the magnitude of average perturbation on the frame. We notice that the magnitude of perturbation on the first and last few frames are larger than that of the middle ones. This means, when the same frame is located at the start or the end part of the input clip, it gets larger distortion.

\begin{figure}[!ht]
	\centering
	\includegraphics[scale=0.3]{images/mag_per_10_untarget.png}
	\caption{Magnitude of perturbation: The x axis is the frame position, and the y axis is the magnitude of average perturbation on the frame. }
	\label{fig:mag_per}
\end{figure}



We further measure the influnece of boundary effect for attack when we have mismatch. \autoref{fig:dismatch_1} shows a mismatch scenario where the way perturbations added on the video stream dismatches the way sliding window chooses input clips. We use offset to measure the extend to which mismatch happens. The experiment result is showed in \autoref{fig:mismatch}. The x axis is the offset between the clip generating perturbation and the clip tested. The y axis is the attack success rate. The results show boundary effect harms the attack a lot if there is dismatch.
 %We measure the harm on target attack, which means, we want the clips to be misclassified to any label. The attack target is set to be the least likely class predicted by the network as suggested by \cite{kurakin2016adversarial, kurakin2016adversarial} The maxinum perturbation on each pixel is set to be 15.The result is showed in \autoref{fig:dismatch_2}. As we can see, target attack harms more from this mismatch problem.

\begin{figure}[!ht]
	\centering
	\includegraphics[scale=0.35]{images/untarget_10_accuracy.png}
	\caption{untarget attack, 10, The x axis is the offset between the clip generating perturbation and the clip tested. The y axis is the attack success rate.}
	\label{fig:dismatch_1}
	\caption{to be explained further}
\end{figure}

%\begin{subfigure}{0.3\textwidth}
%	\includegraphics[scale=0.35]{images/target_15_accuracy.png}
%	\caption{target attack, 15}
%	\label{fig:dismatch_2}
%\end{subfigure}
To conclude, perturbations on same frame are different when locating in different input clips, and this difference affects the attack success rate.


\subsubsection{Input boundaries of video stream are not deterministic}
\label{sec:boundary}

Given a real-time video stream, there is no deterministic boundary for video clips.
To recall (see \autoref{sec:var}), the input for the classifier is chosen by the sliding window. There are three parameters related to the sliding window; window size, starting position, and the stride. Any change on one of these three parameters will result in different input clip and thus different boundaries between video clips. 

Since it is hard for an attacker to know the starting position, it is hard to know in advance where the boundaries of an input clip are. To make things worse, if the stride of sliding is smaller than $w$, one frame can be located in more than one input clips and it will be challenging to deal with these conflicts as showed in \autoref{fig:stride_overlap}.

The fact that current generated perturbations have boundary effect and there is no clear boundary for video task make attack on VAR challenging.

\begin{figure*}[ht!]
	\centering
	\includegraphics[scale=.35]{images/generator_roll.png}
	\caption{This figure provides the architecture of generative adversarial network to produce circular universal perturbations.}
	\label{fig:arc_roll}
\end{figure*}
\begin{figure*}
	\includegraphics[scale=.35]{images/generator_tile.png}
	\caption{This figure provides the architecture of generative adversarial network to produce 2D circular universal perturbations.}
	\label{fig:arc_tile}
\end{figure*}


\subsection{Circular Dual-Purpose Universal Perturbation}
%\label{sec:CDUP}
Based on the dual-purpose universal perturbation (DUP) proposed before, we further propse Circular Dual-Purpose Universal Perturbation (C-DUP) to solve the boundary effect problem.

Suppose the size of sliding window is $w$, then DUP clip $p$ includes $w$ frames of perturbation, which is denoted as $[p_1,p_2, \cdots, p_w]$. Adding perturbation on video stream, we get a perturbation stream $[\cdots,p_{w-1}, p_w,p_1,p_2,\cdots ]$. To guarantee the perturbation stream works no matter how the sliding window chooses clips, we need the perturbation clip $[p_w,r1,\cdots,p_{w-1}]$ to work, also $[p_{w-1},p_w,p_1,\cdots,p_{w-2}]$ and so no. To formulate, we need
all $p_o=Roll(p,o)$ to be valid perturbation for any $o$ where $o$ is the offset by which elements are shifted. 
Therefore, we add one post-process unit which does roll function between the generator and the discriminator, the whole architecture is showed in \autoref{fig:our_arc} and the details about geneartor and the roll unit is showed in \autoref{fig:arc_roll}. 

Same as before, the 3D generator ($G$) takes noise vector as input and output a sequence of perturbations as a perturbation clip %whose size equal to that of the clip input for the C3D model, that is, $16 \times 112 \times 112 \times 3$. 
%maps a noise vector from the latent space to the distribution of perturbation clips ($P$) for a given discriminator ($D$). The architecture of the generator consists of five 3D deconvolution layers. 
Notice that the final layer is followed by a $tanh$ non-linearity and scaling by $\xi$. Doing so restricts the perturbation's range to $[-\xi,\xi]$. 
Following \cite{moosavi2017universal,mopuri2017nag}, the value of $\xi$ is chosen to be 10 in order to add a quasi-imperceptible adverbial perturbation.  The roll unit then rolls the perturbation $p$ by offset in $\{0,1,2,\cdots,w-1\}$.
\autoref{fig:arc_roll} shows with offset euqual to 1, the yellow frame is rolled to the end of the clip. 
Add the rolled perturbation clip to the training input and we get the perturbed input.
As explained before, C3D then take the perturbed input and output the classification score vector.
As before, we want the true class scores for target inputs be low and for non-target inputs be high. Based on the previous optimization problem, we construct this new optimization by adding the roll part.

\begin{comment}
\subsubsection{Discriminator}
Same as \cite{mopuri2017nag}, the discriminator is trained before training the generator and are frozen during the training of the generator.
As presented in \autoref{sec:c3d}, C3D is the state-of-art classifier for human action recognition. Therefore C3D is used as our discriminator. 
To experiment on Jester dataset, we fine-tunde the C3D.
\end{comment}

%Therefore, the final loss function can be formulated as follow.

\begin{equation}
\begin{aligned}
\underset{G}{\text{minimize}} \quad \sum_{o=1,2\cdots w}\{\lambda\times \sum_{t\in T}
{-log[1-Q_c(x_t+Roll(G(z),o))]}\\
+\sum_{s\in S}{-log[Q_c(x_s+Roll(G(z),o))]}\}
\end{aligned}
\end{equation}
In practice, when we training the model, instead of sum over all differernt offests, we choose randomly choose one data set for the sake of efficient.


\subsection{2D Dual-Purpose Universal Perturbation}
We propose a second solution to solve the boundary effect, that is ,add same perturbation on each frame, which can be seen as a special case of C-DUP with $p_1 = p_2 = \cdots = p_w$, where $w$ is a window-size and $p$ refers to perturbation frame. We name this kind of DUP as 2D-DUP because we generate an single-frame perturbation instead of a sequence of perturbation frames as showed in \autoref{fig:arc_tile}. This is a stronger constraint than the circular constraint, which may lead the attack success rate decreases. At the same time, with this constraint, the perturbation generated is simpler and easier to be used in attack. 

%Instead of mapping noise vector from latent space to a perturbation clip, this generator maps the vector to an image perturbation (2D perturbation). The hyper-parameter and architecture is showed in \autoref{fig:gen_tile}. During training, a random vector $z\in R^d$ is sampled from the uniform distribution $U[-1,1]$, which in turn get transformed by G into an image perturbation $p_{2d}$ whose size equal to the frame size (e.g.$112\times112\times3$).

We denote the 2D-DUP as $p_{2d}$, then the perturbation clip is generaed by tile the 2D-DUP $p_{tile} = [p_{2d}, p_{2d}, \cdots, p_{2d}]$ as shown in \autoref{fig:acr_tile}.
The attack objective is same as before, thus we construct this optimization problem as
\begin{equation}
\begin{aligned}
\underset{G_{2D}}{\text{minimize}}\quad \lambda\times \sum_{t\in T}{-log[1-Q_c(x_t+Tile(G_{2D}(z)))]}\\
+\sum_{s\in X-T}{-log[Q_c(x_s+Tile(G_{2D}(z)))]}
\end{aligned}
\end{equation}



\begin{comment}

\subsubsection{How perturbation works?}

As explained in \autoref{sec:c3d}, videos have not only appearance information, but also temporal information.
Appearance information can be simply visualized by plotting RGB images. Here we are interested in whether the perturbations mess up with motion information. 
Optical flow is a common method to measure the motion of image objects between two consecutive frames. It is a 2D vector field (both horizontal and vertical direction) 
where each vector is a displacement vector showing the movement of points from first frame to second. We visualize the optical flow of clean input and perturbed input in 
\autoref{fig:op_compare}.

\autoref{fig:base} shows how color represents the motion. For example, yellow means object moving right and orange means object moving upper right and so on.
The first row in  \autoref{fig:op} represents the original consecutive frames and the other rows shows the optical flow between every two consecutive frames.
The second row  presents the optical flow of a clean Apply Eye Makeup video, we can interpret the optical flow information as following. From the first to the second frame, the hand part first moves down and a little to the left.Then from forth to the fifth frame, the hand part moves right and up.

The third and forth row shows the optical flow of C-DUP and 2D-DUP perturbed frames respectively. It shows that the perturbations do affect motion information in the video.

We then check on other inputs. Two of them are showed in 


\begin{figure*}[t!]
\centering
\begin{subfigure}{0.5\textwidth}
\includegraphics[scale=.3]{images/op_base.png}
\caption{fig:base}
\label{fig:base}
\end{subfigure}
\begin{subfigure}{0.5\textwidth}
\includegraphics[scale=.5]{images/op_compare.png}
\caption{fig$:$compare}
\label{fig:op}
\end{subfigure}
\caption{show the perturbed op}
\label{fig:op_compare}
\end{figure*}

\end{comment}






==> CCS-Sasha 2/threatmodel.tex <==
\section{Threat Model and Datasets}

In this section, we describe our threat model. We also provide a brief overview of the datasets we chose for validating our attack models.

\subsection{Threat model}

We consider a white-box model for our attack, i.e.,
the adversary has access to the training datasets used to train the video classification system,
and has knowledge of the deep neural network model the real-time classification system uses.
We also assume that the adversary is capable of injecting perturbations in the real-time video stream.
In particular, we assume the adversary to be a man-in-the-middle that can
intercept and add perturbations to streaming video \cite{mitm2014videos},
or that it could have previously installed a malware that is able to add perturbation
prior to classification \cite{malware2016zdnet}.

We assume that the goal of the adversaries is to launch stealthily attacks,
i.e., they want the system to only misclassify the malicious actions
without affecting the recognition of the other actions.
So, we consider two attack goals.
\textit{First}, given a target class, we want all the clips from this class
to be misclassified by the real-time video classifier.
\textit{Second}, for all the clips from other (non-target) classes,
we want the classifier to correctly classify them.

% \footnote{{\color{black} Here,
% we assume that a either a previously generated malware adds the perturbation prior to classification
% or that the adversary is a man-in-the-middle inserting perturbations in the video in between the
% video capture system and the classifier.}}

%\reminder{[How to inject this perturbation -> man-in-the-middle attack in the network to inject the videos, there can be malware in the system injecting these perturbations in the videos.]}
%We would explore black-box attack a little. The attack goal is to make one or more classes of suspicious actions not to be recognized and at the same time, the attack need to be as stealthy as possible, which means, the attack should affect the recognition of the other actions as least as possible.

\subsection{Our datasets} %[made modification for the whole section]}
\label{sec:dataset}
We use the human action recognition dataset UCF-101 \cite{soomro2012ucf101} and the hand gesture recognition dataset 20BN-JESTER dataset (Jester) \cite{jester2016} to validate our attacks on 
video classification systems. We use these two datasets because they represent two kinds of classification, i.e., coarse-gained and fine-grained action classification. 

\heading{The UCF 101 dataset:}
The UCF 101 dataset used in our experiments is the standard dataset collected from Youtube. It includes 13320 videos from 101 human action categories (e.g., applying lipstick, biking, blow drying hair, 
cutting in the kitchen etc.). The videos collected in this dataset have variations in camera motion, appearance, background, illumination conditions etc. Given the diversity it provides, we consider the dataset to validate the feasibility of our attack model on coarse-gained actions. 
There are three different (pre-existing) splits \cite{soomro2012ucf101} in the dataset; we use split 
1 for both training and testing, in our experiments. The training set includes 9,537 video clips and the testing set includes 3,783 video clips.
%{\color{blue}more details about training, validation, and test set}

\heading{The Jester dataset:}
The 20BN-JESTER dataset (Jester)  is a recently collected dataset with hand gesture videos. These videos are recorded by crowd-source workers performing 27 kinds of gestures (e.g., sliding hand left, sliding two fingers left, zooming in with full hand, zooming out with full hand etc.). We use this dataset to validate our attack with regards to fine-grained actions.
Since this dataset does not currently provide labels for the testing set, 
we use the validation set as our testing set (i.e., apply our perturbations on the validation set). 
The training set has 148,092 short video clips and our testing set has 14,787 short video clips.

%Figure belonging to boundary problem



==> temporaldimension_shasha.tex <==
\section{The time machine: handling the temporal dimension}
\label{sec:temporal}
In this section, we discuss why directly applying existing methods to generate perturbation for video stream do not work, and propose our novel perturbations to solve the problem.
\begin{figure}%[t]
	\centering
	\begin{subfigure}{0.5\textwidth}
		\includegraphics[scale=.4]{images/explain_mismatch.png}
		\subcaption{mismatch}
		\label{fig:mismatch}    
	\end{subfigure}
	\begin{subfigure}{0.5\textwidth}
		\includegraphics[scale=.4]{images/explain_stride_overlap.png}
		\subcaption{overlap}
		\label{fig:stride_overlap}   
	\end{subfigure}
	\caption{sliding window}
	\label{fig:sliding_window}
\end{figure}
\subsection{Motivation}

\subsubsection{Boundary effect existing in perturbations}
Perturbation is generated by optimising the input of the DNNs toward misclassication. Since the input for the video classifier is a sequence of frames (we mention it as clip afterward), the perturbation is generated driven by input clips.
However, when a frame is located in different clip, the perturbation generated for it are different. This means the boundaries of the clips will have an effect on the perturbations generated. We name this as boundary problem. To elaborate, suppose a video stream $\{ ...,f_{i-2}, f_{i-1}, f_i,
f_{i+1},f_{i+2}, ...\}$, the perturbation on $f_i$ generating by choosing clip [$f_{i}, f_{i+1}, \cdots, f_{i+w-1}$] is different from the one generated by clip [$[_{i-1}, f_{i}, f_{i+1} \cdots, f_{i+w-2}]$].
Therefore, whether the boundary of input clips chosen between $f_{i-1}$ and $f_{i}$ or between $f_{i-2}$ and $f_{i-1}$ influences the perturbation on $f_i$, and also on the other frames.

We use the existing popular perturbation generation method basic iteration~\cite{kurakin2016adversarial}
%four currently existing popular perturbation generation methods namely, fast gradient~\cite{goodfellow2014explaining}, basic iteration~\cite{kurakin2016adversarial}, CarliniWagnerL2~\cite{carlini2017towards}, and saliency map \cite{papernot2016limitations} 
{\color{blue} may get results from other existing attack methods if time allowed}
to showcase the boundary effect problem.
We use the API from CleverHands \cite{papernot2016cleverhans}, an Python libary to generate perturbations for all the videos from UCF-101 testing set based on C3D model (see \autoref{sec:c3d}). The maximum perturbation on each pixel is set to be 10 (the image is represent in [0,255]). The step size for each attack iteration is set to be 1 and the number of attack iterations is set to be 14. We set the attack to be untargeted attack, which means, we want the clips to be misclassified to any label.

We then test the correlation between these different perturbations on the same frames. Averaged correlation matrix is shown in \autoref{fig:corre}. Both the row and the column represents the location of the frame and the value showed in row $r$ and column $c$ means the normalized correlation between the perturbation generated when it is the $r$th frame and the $c$th frame in the input clips. The result show that the perturbations on the same frames are different quantitively.  

\begin{figure}[!ht]
	\centering
	\includegraphics[scale=0.3]{images/correlation_untarg_10.png}
	\caption{correlation matrix,to be explained further}
	\label{fig:corre}
\end{figure}

We measure the average magnitude of perturbations on different locations as shown in \autoref{fig:mag_per}. The x axis is the frame position, and the y axis is the magnitude of average perturbation on the frame. We notice that the magnitude of perturbation on the first and last few frames are larger than that of the middle ones. This means, when the same frame is located at the start or the end part of the input clip, it gets larger distortion.

\begin{figure}[!ht]
	\centering
	\includegraphics[scale=0.3]{images/mag_per_10_untarget.png}
	\caption{Magnitude of perturbation: The x axis is the frame position, and the y axis is the magnitude of average perturbation on the frame. }
	\label{fig:mag_per}
\end{figure}



We further measure the influnece of boundary effect for attack when we have mismatch. \autoref{fig:dismatch_1} shows a mismatch scenario where the way perturbations added on the video stream dismatches the way sliding window chooses input clips. We use offset to measure the extend to which mismatch happens. The experiment result is showed in \autoref{fig:mismatch}. The x axis is the offset between the clip generating perturbation and the clip tested. The y axis is the attack success rate. The results show boundary effect harms the attack a lot if there is dismatch.
 %We measure the harm on target attack, which means, we want the clips to be misclassified to any label. The attack target is set to be the least likely class predicted by the network as suggested by \cite{kurakin2016adversarial, kurakin2016adversarial} The maxinum perturbation on each pixel is set to be 15.The result is showed in \autoref{fig:dismatch_2}. As we can see, target attack harms more from this mismatch problem.

\begin{figure}[!ht]
	\centering
	\includegraphics[scale=0.35]{images/untarget_10_accuracy.png}
	\caption{untarget attack, 10, The x axis is the offset between the clip generating perturbation and the clip tested. The y axis is the attack success rate.}
	\label{fig:dismatch_1}
	\caption{to be explained further}
\end{figure}

%\begin{subfigure}{0.3\textwidth}
%	\includegraphics[scale=0.35]{images/target_15_accuracy.png}
%	\caption{target attack, 15}
%	\label{fig:dismatch_2}
%\end{subfigure}
To conclude, perturbations on same frame are different when locating in different input clips, and this difference affects the attack success rate.


\subsubsection{Input boundaries of video stream are not deterministic}
\label{sec:boundary}

Given a real-time video stream, there is no deterministic boundary for video clips.
To recall (see \autoref{sec:var}), the input for the classifier is chosen by the sliding window. There are three parameters related to the sliding window; window size, starting position, and the stride. Any change on one of these three parameters will result in different input clip and thus different boundaries between video clips. 

Since it is hard for an attacker to know the starting position, it is hard to know in advance where the boundaries of an input clip are. To make things worse, if the stride of sliding is smaller than $w$, one frame can be located in more than one input clips and it will be challenging to deal with these conflicts as showed in \autoref{fig:stride_overlap}.

The fact that current generated perturbations have boundary effect and there is no clear boundary for video task make attack on VAR challenging.

\begin{figure*}[ht!]
	\centering
	\includegraphics[scale=.35]{images/generator_roll.png}
	\caption{This figure provides the architecture of generative adversarial network to produce circular universal perturbations.}
	\label{fig:arc_roll}
\end{figure*}
\begin{figure*}
	\includegraphics[scale=.35]{images/generator_tile.png}
	\caption{This figure provides the architecture of generative adversarial network to produce 2D circular universal perturbations.}
	\label{fig:arc_tile}
\end{figure*}


\subsection{Circular Dual-Purpose Universal Perturbation}
%\label{sec:CDUP}
Based on the dual-purpose universal perturbation (DUP) proposed before, we further propse Circular Dual-Purpose Universal Perturbation (C-DUP) to solve the boundary effect problem.

Suppose the size of sliding window is $w$, then DUP clip $p$ includes $w$ frames of perturbation, which is denoted as $[p_1,p_2, \cdots, p_w]$. Adding perturbation on video stream, we get a perturbation stream $[\cdots,p_{w-1}, p_w,p_1,p_2,\cdots ]$. To guarantee the perturbation stream works no matter how the sliding window chooses clips, we need the perturbation clip $[p_w,r1,\cdots,p_{w-1}]$ to work, also $[p_{w-1},p_w,p_1,\cdots,p_{w-2}]$ and so no. To formulate, we need
all $p_o=Roll(p,o)$ to be valid perturbation for any $o$ where $o$ is the offset by which elements are shifted. 
Therefore, we add one post-process unit which does roll function between the generator and the discriminator, the whole architecture is showed in \autoref{fig:our_arc} and the details about geneartor and the roll unit is showed in \autoref{fig:arc_roll}. 

Same as before, the 3D generator ($G$) takes noise vector as input and output a sequence of perturbations as a perturbation clip %whose size equal to that of the clip input for the C3D model, that is, $16 \times 112 \times 112 \times 3$. 
%maps a noise vector from the latent space to the distribution of perturbation clips ($P$) for a given discriminator ($D$). The architecture of the generator consists of five 3D deconvolution layers. 
Notice that the final layer is followed by a $tanh$ non-linearity and scaling by $\xi$. Doing so restricts the perturbation's range to $[-\xi,\xi]$. 
Following \cite{moosavi2017universal,mopuri2017nag}, the value of $\xi$ is chosen to be 10 in order to add a quasi-imperceptible adverbial perturbation.  The roll unit then rolls the perturbation $p$ by offset in $\{0,1,2,\cdots,w-1\}$.
\autoref{fig:arc_roll} shows with offset euqual to 1, the yellow frame is rolled to the end of the clip. 
Add the rolled perturbation clip to the training input and we get the perturbed input.
As explained before, C3D then take the perturbed input and output the classification score vector.
As before, we want the true class scores for target inputs be low and for non-target inputs be high. Based on the previous optimization problem, we construct this new optimization by adding the roll part.

\begin{comment}
\subsubsection{Discriminator}
Same as \cite{mopuri2017nag}, the discriminator is trained before training the generator and are frozen during the training of the generator.
As presented in \autoref{sec:c3d}, C3D is the state-of-art classifier for human action recognition. Therefore C3D is used as our discriminator. 
To experiment on Jester dataset, we fine-tunde the C3D.
\end{comment}

%Therefore, the final loss function can be formulated as follow.

\begin{equation}
\begin{aligned}
\underset{G}{\text{minimize}} \quad \sum_{o=1,2\cdots w}\{\lambda\times \sum_{t\in T}
{-log[1-Q_c(x_t+Roll(G(z),o))]}\\
+\sum_{s\in S}{-log[Q_c(x_s+Roll(G(z),o))]}\}
\end{aligned}
\end{equation}
In practice, when we training the model, instead of sum over all differernt offests, we choose randomly choose one data set for the sake of efficient.


\subsection{2D Dual-Purpose Universal Perturbation}
We propose a second solution to solve the boundary effect, that is ,add same perturbation on each frame, which can be seen as a special case of C-DUP with $p_1 = p_2 = \cdots = p_w$, where $w$ is a window-size and $p$ refers to perturbation frame. We name this kind of DUP as 2D-DUP because we generate an single-frame perturbation instead of a sequence of perturbation frames as showed in \autoref{fig:arc_tile}. This is a stronger constraint than the circular constraint, which may lead the attack success rate decreases. At the same time, with this constraint, the perturbation generated is simpler and easier to be used in attack. 

%Instead of mapping noise vector from latent space to a perturbation clip, this generator maps the vector to an image perturbation (2D perturbation). The hyper-parameter and architecture is showed in \autoref{fig:gen_tile}. During training, a random vector $z\in R^d$ is sampled from the uniform distribution $U[-1,1]$, which in turn get transformed by G into an image perturbation $p_{2d}$ whose size equal to the frame size (e.g.$112\times112\times3$).

We denote the 2D-DUP as $p_{2d}$, then the perturbation clip is generaed by tile the 2D-DUP $p_{tile} = [p_{2d}, p_{2d}, \cdots, p_{2d}]$ as shown in \autoref{fig:acr_tile}.
The attack objective is same as before, thus we construct this optimization problem as
\begin{equation}
\begin{aligned}
\underset{G_{2D}}{\text{minimize}}\quad \lambda\times \sum_{t\in T}{-log[1-Q_c(x_t+Tile(G_{2D}(z)))]}\\
+\sum_{s\in X-T}{-log[Q_c(x_s+Tile(G_{2D}(z)))]}
\end{aligned}
\end{equation}



\begin{comment}

\subsubsection{How perturbation works?}

As explained in \autoref{sec:c3d}, videos have not only appearance information, but also temporal information.
Appearance information can be simply visualized by plotting RGB images. Here we are interested in whether the perturbations mess up with motion information. 
Optical flow is a common method to measure the motion of image objects between two consecutive frames. It is a 2D vector field (both horizontal and vertical direction) 
where each vector is a displacement vector showing the movement of points from first frame to second. We visualize the optical flow of clean input and perturbed input in 
\autoref{fig:op_compare}.

\autoref{fig:base} shows how color represents the motion. For example, yellow means object moving right and orange means object moving upper right and so on.
The first row in  \autoref{fig:op} represents the original consecutive frames and the other rows shows the optical flow between every two consecutive frames.
The second row  presents the optical flow of a clean Apply Eye Makeup video, we can interpret the optical flow information as following. From the first to the second frame, the hand part first moves down and a little to the left.Then from forth to the fifth frame, the hand part moves right and up.

The third and forth row shows the optical flow of C-DUP and 2D-DUP perturbed frames respectively. It shows that the perturbations do affect motion information in the video.

We then check on other inputs. Two of them are showed in 


\begin{figure*}[t!]
\centering
\begin{subfigure}{0.5\textwidth}
\includegraphics[scale=.3]{images/op_base.png}
\caption{fig:base}
\label{fig:base}
\end{subfigure}
\begin{subfigure}{0.5\textwidth}
\includegraphics[scale=.5]{images/op_compare.png}
\caption{fig$:$compare}
\label{fig:op}
\end{subfigure}
\caption{show the perturbed op}
\label{fig:op_compare}
\end{figure*}

\end{comment}





